Visual Relationship Detection with Internal and External Linguistic Knowledge Distillation

Understanding visual relationships involves identifying the subject, the object, and a predicate relating them. We leverage the strong correlations between the predicate and the (subj,obj) pair (both semantically and spatially) to predict the predicates conditioned on the subjects and the objects. Modeling the three entities jointly more accurately reflects their relationships, but complicates learning since the semantic space of visual relationships is huge and the training data is limited, especially for the long-tail relationships that have few instances. To overcome this, we use knowledge of linguistic statistics to regularize visual model learning. We obtain linguistic knowledge by mining from both training annotations (internal knowledge) and publicly available text, e.g., Wikipedia (external knowledge), computing the conditional probability distribution of a predicate given a (subj,obj) pair. Then, we distill the knowledge into a deep model to achieve better generalization. Our experimental results on the Visual Relationship Detection (VRD) and Visual Genome datasets suggest that with this linguistic knowledge distillation, our model outperforms the state-of-the-art methods significantly, especially when predicting unseen relationships (e.g., recall improved from 8.45% to 19.17% on VRD zero-shot testing set).

==> 906 2/Experiment.tex <==
\section{Experiments}\label{exp}
% We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
We evaluate our method on Visual Relationship Detection \cite{VRD} and Visual Genome \cite{VG} datasets for three tasks:
\textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
\textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
\textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.

% 1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
% 2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
% 3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
%   \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
%   \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \end{itemize}

Both datasets have a zero-shot testing set that contains relationships that never occur in the training data. We evaluate on the zero-shot sets to demonstrate the generalization improvements brought by linguistic knowledge distillation.

\textbf{Implementation Details.} We use VGG-16 \cite{VGG} to learn the visual representations of the BB-Union of two objects. 
% For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. 
% For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, 
We use a pre-trained word2vec \cite{word2vec}  model to project the subjects and objects into vector space, and the final semantic representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\textbf{{Evaluation Metric.}} We follow \cite{VRD,UIUC} using Recall@$n$ (R@$n$) as our evaluation metric (mAP metric would mistakenly penalize true positives because annotations are not exhaustive).
For two detected objects, multiple predicates are predicted with different confidences. The standard R@$n$ metric ranks all predictions for all object pairs in an image and compute the recall of top $n$. However, instead of computing recall based on all predictions, \cite{VRD} considers only the predicate with highest confidence for each object pair. 
Such evaluation is more efficient and forced the diversity of object pairs. 
However, multiple predicates can correctly describe the same object pair and the annotator only chooses one as ground truth, \eg, when describing a person ``next to" another person, predicate ``near" is also plausible.
So we believe that a good predicted distribution should have high probabilities for all plausible predicate(s) and probabilities close to 0 for remaining ones.  Evaluating only the top prediction per object pair may mistakenly penalize correct predictions since annotators have bias over several plausible predicates. 
So we treat the number of chosen predictions per object pair ($k$) as a hyper-parameter, and report R@$n$ for different $k$'s to compare with other methods \cite{VRD,UIUC,VisualPhrase}. Since the number of predicates is 70, $k=70$ is equivalent to evaluating all predictions \wrt two detected objects. 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
% 1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
% 2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial feature; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them. Part 1 uses the VRD training images; Part 2 uses the training images in VRD \cite{VRD} and images of Visual Genome (VG) \cite{VG} dataset.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection, R@100,k=1 and R@50,k=1 are equivalent (also observed in \cite{VRD}) because there are not enough objects in ground truth to produce over 50 pairs.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20
\tablefootnote{\label{70}The recall of different k's are not reported in \cite{VRD}.We calculate those recall values using their code.}          
& 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 34.82     & 83.15       & 70.02    & 12.75     & 69.42       & 47.84   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 37.15     & 83.78       & 70.75   & 13.44     & 69.77       & 49.01    \\
U+W+L:S               & 42.98     & 84.94       & 71.83  & 13.89       & 72.53       & 51.37     \\
U+W+L:T               & 52.96     & 88.98       & 83.26   & 7.81          & 40.15      & 32.62   \\\hdashline
U+SF                 &36.33           & 83.68       & 69.87  & 14.33     & 69.01       & 48.32    \\
U+SF+L:S                       & 41.06     & 84.81       & 71.27    & 15.14          & 72.72       & 51.62  \\
U+SF+L:T               & 51.67     & 87.71       & 83.84     & 8.05          & 41.51       & 32.77    \\ \hdashline
U+W+SF                   & 41.33     & 84.89       & 72.29  & 14.13         & 69.41       & 48.13    \\
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & \textbf{16.98}       & \textbf{74.65}       & \textbf{54.20}    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81    \\
U+W+SF+L: T+S    & \textbf{55.16}     & \textbf{94.65}       & \textbf{85.64}    & -          & -       & -  \\
\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}
                                              & & &  &                      \\
Baseline: U                                           & 36.97     & 84.49  & 70.19   & 13.31     & 70.56  & 50.34     \\
U+W+SF                     & 42.08     & 85.89       & 72.83   & 14.51          & 70.79       & 50.64     \\
U+W+SF+L: S             & 48.61      & 87.15       & 75.45    & 17.16          & 75.26       & 55.41     \\
U+W+SF+L: T             & 54.61     & 90.09       & 82.97       & 9.23          & 43.21       & 33.40  \\
U+W+SF+L: T+S               & 55.67     &95.19      & 86.14    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}


\begin{figure*}[t]
\centering     %%% not \center
\subfigure[Seen relationships]{\label{v}\includegraphics[width=140mm]{images/Camera_ready_v1.pdf}}

\subfigure[Zero-shot Relationships]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of predicate detection results: ``Data-driven" denotes the baseline using BB-Union; ``LK only" denotes the baseline using only the linguistic knowledge without looking at the image; ``Full model student" denotes the student network with U+W+SF features; ``Full model teacher" denotes the teacher network with U+W+SF features.}
\end{figure*}

\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
% Our method models the conditional probability $P(pred|subj,obj,B_s,B_o,I)$. 
% So, w
We first evaluate it on predicate prediction (as in \cite{VRD}).
% Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. 
Since \cite{UIUC,VIPCNN,RL} do not report results of predicate prediction, we compare our results with ones in \cite{VRD, VisualPhrase}. 

Part 1 of Table \ref{P_VRD} shows the results of linguistic knowledge distillation with different sets of features in our deep neural networks. In addition to the data-driven baseline ``Baseline: U only", we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". The ``Visual Phrases" method \cite{VisualPhrase} trains deformable parts models for each relationship; ``Joint CNN" \cite{Rcnn} trains a 270-way CNN to predict the subject, object and predicate together. The visual only model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in training, we use the student network's output. 

\textbf{End-to-end CNN training with semantic and spatial representations.} Comparing our baseline, which uses the same visual representation (BB-Union) as \cite{VRD}, and the ``VRD-V only" model, our huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 34.82\%) reveals that the end-to-end training with soft-max prediction outperforms extracting features from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding the semantic representation and the spatial features improves the predictive power and generalization of the data-driven model\footnote{More analysis on using different combinations of features can be found in the supplementary materials.}.






To demonstrate the effectiveness of LK-distillation, we compare the results of using different combinations of features with/without using LK-distillation. In Part 1 of Table \ref{P_VRD}, we train and test our model on only the VRD dataset, and use the training annotation as our linguistic knowledge. 
\textit{``Linguistic knowledge only" baseline} (``Baseline: L only") itself has a strong predictive power and it outperforms the state-of-the-art method \cite{VRD} by a large margin (\eg, 51.34\%  vs. 47.87\% for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without looking at the images leads to very poor performance on the zero-shot set of VRD, which explains the poor generalization of ``Baseline: L only" method and addresses the need for combining both data-driven and knowledge-based methods as the LK-distillation framework we propose does.



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 0.07             & 0.04           & -    & - & - & -   & -& -& -& -& -   \\
Joint CNN  \cite{Rcnn}           & 0.09             & 0.07           & -    & - & - & - & 0.09    & 0.07 & - & -& -    & -      \\
% VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & -                      & -       & -                      & -               &14.70                  & 13.86                  & -                      & -            & -                    & -          \\
VRD - V only  \cite{VRD}           & 2.61             & 2.24           & -    & - & - & - & 1.85    & 1.58 & - & -& -    & -      \\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                     & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\
VIP-CNN   \cite{VIPCNN}       & \textbf{27.91}                      & 22.78                      & -                  & -                & --                      & --  & 20.01                      & 17.32                      & -                 & -         & --                      & --         \\
VRL   \cite{RL}       & 22.60                     & 21.37                      & -                 & -               & --                      & --  & 20.79                      & 18.19                      & -                  & -        & --                      & --         \\\hdashline
U+W+SF+L: S      & 19.98 & 19.15 & 25.16 & 22.95 & 25.54	& 22.59 & 17.69 & 16.57 & 27.98 & 19.92 &28.94	&20.12\\
U+W+SF+L: T      & 23.57 & 22.46 & 29.14 & 25.96 &29.09	&25.86 & 20.61 & 18.56 & 29.41 & 21.92 &31.13	&21.98\\
U+W+SF+L: T+S  & 24.03 & \textbf{23.14} & \textbf{29.76} & \textbf{26.47} &\bf29.43	&\bf26.32 & \textbf{21.34} & \textbf{19.17} & \textbf{29.89} & \textbf{22.56} &\bf 31.89	&\bf22.68\\

\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 20.32 & 19.96 & 25.71 & 23.34 & 25.97	& 22.83 & 18.32 & 16.98 & 28.24 & 20.15 &29.85	&21.88\\
U+W+SF+L: T      & 23.89 & 22.92 & 29.82 & 26.34 &29.97	&26.15 & 20.94 & 18.93 & 29.95 & 22.62 &31.78	&22.65\\
U+W+SF+L: T+S     & 24.42 & 23.51 & 30.13 & 26.73 &30.01 &26.58 & 21.72 & 19.68 & 30.45 & 22.84 &32.56	&23.18\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&&&&&&&\\

% VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & -                     & -    & -                      & -                  & 3.52                  & 3.13                  & -                      & -      & -                     & -                \\
VRD - V only  \cite{VRD}           & 1.12             & 0.95           & -    & - & - & - & 0.78    & 0.67 & - & -& -    & -      \\
VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\
% VIP-CNN   \cite{VIPCNN}       & -                     & -                    & -                  & -                & --                      & --  & --                      & --                      & -                 & -         & --                      & --         \\
VRL   \cite{RL}       & 10.31                    & 9.17                      & -                 & -               & --                      & --  & 8.52                      & 7.94                      & -                  & -        & --                      & --         \\
\hdashline
U+W+SF+L: S   & \textbf{10.89} & \textbf{10.44} & \textbf{17.24} & \textbf{13.01} &\bf 17.24	&\bf 12.96 & \textbf{9.14} & \textbf{8.89} & \textbf{16.15} & \textbf{12.31} &\bf 15.89	&\bf 12.02\\ 	
U+W+SF+L: T      & 6.71 & 6.54 & 11.27 & 9.45 &9.84	&7.86 & 6.44 & 6.07 & 9.71 & 7.82 &10.21	&8.75\\
\midrule
   
\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 11.23 & 10.87 & 17.89 & 13.53 & 17.88	& 13.41 & 9.75 & 9.41 & 16.81 & 12.72 &16.37	&12.29\\
U+W+SF+L: T      & 7.03 & 6.94 & 11.85 & 9.88 &10.12	&8.97 & 6.89 & 6.56 & 10.34 & 8.23 &10.53	&9.03\\

\bottomrule


\end{tabular}
\end{table*}



\textbf{The benefit of LK distillation} is visible across all feature settings: the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models significantly (\eg, R@100/50, k=1 is improved from 37.15\% to 42.98\% for ``U+W" features on the entire VRD test set).
% On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
% There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in the training data; the other is that although the linguistic prior is powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on the zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin.
% (\eg, 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher is the final output, we achieve better predictive power by combining both: we use the teacher network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining. The setting ``U+W+SF+LK: T+S" performs the best. 
% One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. 
Fig. \ref{v} and \ref{vz} show a visualization of different methods.

\subsubsection{Phrase and Relationship Detection}
To enable fully automatic phrase and relationship detection, we train a Fast R-CNN detector \cite{fastRCNN} using VGG-16 for object detection. Given the confidence scores of detected each detected object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Fig. \ref{fig:system} to obtain the predicted predicate distribution for each pair of objects. According to Eq. \ref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. We also adopt the triplet NMS in \cite{VIPCNN} to remove redundant detections. To compare with \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report recall. In addition, we report the full recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Part 1 of Tables \ref{Detection} and \ref{Detection_Zero}. Our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} significantly on both entire testing set and zero-shot setting. The observations about student and teacher networks are consistent with predicate prediction evaluation. 
We also compare our method with the very recently introduced ``VIP-CNN" in \cite{VIPCNN} and ``VRL" \cite{RL} and achieve better or comparable results. For phrase detection, we achieve better results than \cite{RL} and get similar result for R@50 to \cite{VIPCNN}. One possible reason that \cite{VIPCNN} gets better result for R@100 is that they jointly model the object and predicate detection while we use an off-the-shelf detector.
% and focus more on predicting predicates.
% \footnote{We aware the existence of the two new paper \cite{RL,VIPCNN} right before the submission deadline. We are communicating with the authors to ask for their detections so we may combine our methods with theirs to get etter results}. 
For relationship detection, we outperform both methods, especially on the zero-shot set.
% (\cite{VIPCNN} does not report results on the zero-shot set).  
% However, as we discussed, different choices of ``k" will affect the number dramatically, and paper \cite{UIUC} who claimed they used the same experiment metric with \cite{VRD} has chosen different k. Since \cite{RL,VIPCNN} did not reveal the k they chose, so we assume they chose k=1. 

% Additionally, when comparing the results of predicate and relationship prediction, the large performance gain (5.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental object detection task.

% \vspace{-2mm}
\subsection{Evaluation on Visual Genome Dataset}
We also evaluate predicate detection on Visual Genome (VG) \cite{VG}, the largest dataset that has visual relationship annotations. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships whose predicates and objects occur in the VRD dataset. We conduct a similar evaluation on the dataset (99,864 relationship instances in training and 19,754 in testing; 2,056 relationship test instances are never seen in training). We use the linguistic knowledge extracted from VG and report predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar behavior as on the VRD dataset---LK distillation regularizes the deep model and improves its generalization. We conduct another experiment in which images from Visual Genome dataset augment the training set of VRD and evaluate on the VRD test set. From the Part 2 of Tables \ref{P_VRD}, \ref{Detection} and \ref{Detection_Zero}, we observe that training with more data leads to only marginal improvement over almost all baselines and proposed methods. However, for all experimental settings, our LK distillation framework still brings significant improvements, and the combination of the teacher and student networks still yields the best performance. This reveals that incorporating additional knowledge is more beneficial than collecting more data\footnote{Details can be found in the supplementary materials.}. 

\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset. Notations are the same as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 37.81    & 82.05    & 81.41    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.92    & 86.81    & 84.92    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. Part 1 uses the LK from VRD dataset; Part 2 uses the LK from VG dataset; Part 3 uses the LK from both VRD and VG dataset. Part 4 uses the LK from parsing Wikipedia text; Part 5 uses the LK from from both VRD dataset and Wikipedia. Notations are the same as as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
Part 1 LK: VRD  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & 16.98       & 74.65       & 54.20    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81     \\\midrule
Part 2 LK: VG & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 16.88   & 72.29    & 52.51   \\
U+W+SF+L: T         & 51.54    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{Part 3 LK: VRD+VG} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 17.21    & 74.89   & 54.65   \\
U+W+SF+L: T         & \textbf{54.82}    & \textbf{90.63}    & \textbf{83.97}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{Part 4 LK: Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{Part 5 LK: VRD+Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.94   & 87.11   & 77.79    & \textbf{19.17}    & \textbf{76.42}    & \textbf{56.81}   \\
U+W+SF+L: T         & 54.06    & 88.93   & 81.78    & 9.65     & 42.24   & 34.61  \\\bottomrule
\end{tabular}
\end{table}

\subsection{Distillation with External Knowledge}
The above experiments show the benefits of extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
% However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
However, training annotations only represent a small portion of all possible relationships and do not necessarily represent the real world distribution, which has a long tail.
For unseen long-tail relationships in the VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated dataset. 
In Table \ref{VRD_use_VG_Stat}, we show predicate detection results on the VRD test set using our linguistic knowledge distillation framework with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy one obtained from Wikipedia, leads to bad performance. 
However, interestingly, although the external knowledge can be very noisy (Wikipedia) and has a different distribution when compared with the VRD dataset (Visual Genome), the performance of the teacher network using external knowledge is much better than using only the internal knowledge (Part 1). 
This suggests that by properly distilling external knowledge, our framework obtains both good predictive power on the seen relationships and better generalization on unseen ones. 
% To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
% After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
% The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
% We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. We observe that by distilling external knowledge \textit{and} the internal one, we improve generalization significantly (\eg, LK from Wikipedia boosts the recall to 19.17\% on the zero-shot set) while maintaining good predictive power on the entire test set.


\begin{figure}[!t]
\centering
  \includegraphics[height=3cm]{images/I_N}
  \caption{Performance with varying sizes of training examples. ``Our Method" denotes the student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text. ``VRD-Full" is the full model in \cite{VRD}.}
\label{fig:im}
\end{figure}

% \vspace{-2mm}

Fig. \ref{fig:im} shows the comparison between our student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text (denoted as ``Our Method") and the full model in \cite{VRD} (denoted as ``VRD-Full"). We observe that our method significantly outperforms the existing method, especially for the zero-shot (relationships with 0 training instance) and the few-shot setting (relationships with few training instances, \eg, $\le10$). By distilling linguistic knowledge into a deep model, our data-driven model improves dramatically, which is hard to achieve by only training on limited labeled images.



% By properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
% By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (\eg \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.











==> 906 2/K.tex <==
\section{Our Approach}
A straightforward way to predict relationship predicates is to train a CNN on the union of the two bounding boxes that contain the two objects of interest as the visual input, fuse semantic features (that encode the object categories) and spatial features (that encode the relative positions of the objects) with the CNN features  (that encode the appearance of the objects), and feed them into a fully connected (FC) layer to yield an end-to-end prediction framework. However, the number of \threetup{subj}{pred}{obj} tuples is very large and the parameter space of the end-to-end CNN would be huge. 
While the subject, predicate, and object are not statistically independent, a CNN would require a massive amount of data to discover the dependence structure while also learning the mapping from visual features to semantic relationships.
% It is hard to collect sufficient data for the large number of relationships. 
To avoid over-fitting and achieve better predictive power without increasing the amount of visual training data, additional information is needed to help regularize the training of the CNN.

Figure \ref{fig:system} summarizes our proposed model. Given an image, we extract three input components: the cropped images of the union of the two detected objects (BB-Union); the semantic object representations obtained from the object category confidence score distributions obtained from the detector; and the spatial features (SF) obtained from pairs of detected bounding boxes.
We concatenate VGG features, semantic object vectors, and the spatial feature vectors, then train another FC layer using the ground truth label (GT) and the linguistic knowledge to predict the predicate. Unlike \cite{VRD}, which used the VGG features to train a linear model, our training is end-to-end without fixing the VGG-net. Following \cite{eric1,eric2}, we call the data-driven model the ``student", and the linguistic knowledge regularized model the ``teacher".

\subsection{Linguistic Knowledge Distillation}
\subsubsection{Preliminary: Incorporating Knowledge in DNNs}
The idea of incorporating additional information in DNNs has been exploited recently \cite{hinton,eric1,eric2}. We adapted Hu \emph{et al.}'s teacher-student framework \cite{eric1,eric2} to distill linguistic knowledge in a data-driven model. The teacher network is constructed by optimizing the following criterion:
\begin{equation}
\label{optimization}
\min_{t \in T}\text{KL}(t(Y)|| s_{\phi}(Y|X)) - C \mathbb{E}_t[L(X,Y)],
\end{equation}
where $t(Y)$ and $s_{\phi}(Y|X)$ are the prediction results of the teacher and student networks; C is a balancing term; $\phi$ is the parameter set of the student network; $L(X,Y)$ is a general constraint function that has high values to reward the predictions that meet the constraints and penalize the others. $\text{KL}$ measures the KL-divergence of teacher's and student's prediction distributions. The closed-form solution of the optimization problem is:  
\begin{equation}
\label{teacher_Network}
t(Y) \propto s(Y|X)\text{exp}(CL(X,Y))~.
\end{equation}
The new objective which contains both ground truth labels and the teacher network is defined as:
\begin{equation}
\label{objective}
\min_{\phi \in \Phi } \frac{1}{n} \sum_{i=1}^{n}\alpha l(s_i,y_i)+(1-\alpha)l(s_i,t_i),
\end{equation}
where $s_i$ and $t_i$ are the student's and teacher's predictions for sample $i$; $y_i$ is the ground truth label for sample $i$; $\alpha$ is a balancing term between ground truth and the teacher network. $l$ is the loss function. More details can be found in \cite{eric1,eric2}.

\subsubsection{Knowledge Distillation for Visual Relationship Detection}
Linguistic knowledge is modeled by a conditional probability that encodes the strong correlation between the pair of objects \twotup{subj}{obj} and the predicate that humans tend to use to describe the relationship between them:
\begin{equation}
\label{language_knowledge}
L(X,Y)=\log P(pred|subj,obj),
\end{equation}
where X is the input data and $Y$ is the output distribution of the student network. $P(pred|subj,obj)$ is the conditional probability of a predicate given a fixed \twotup{subj}{obj} pair in the obtained linguistic knowledge set.

By solving the optimization problem in Eq.~\ref{optimization}, we construct a teacher network that is close to the student network, but penalizes a predicted predicate that is unlikely given the fixed \twotup{subj}{obj} pairs. The teacher's output can be viewed as a projection of the student's output in the solution space constrained by linguistic knowledge. For example, when predicting the predicate between a ``plate" and a ``table", given the subject (``plate") and the object (``table"), and the conditional probability $P(pred|plate,table)$, the teacher will penalize unlikely predicates, (\eg, ``in") and reward likely ones (\eg, ``on"), helping the network avoid portions of the parameter space that lead to poor solutions. 
% For example, given two bounding boxes of the subject (red) and object (blue) shown in Figure \ref{fig:example}, it is hard to determine which predicate is correct, and while a network could learn to make this prediction by relying only on the pixels within those boxes, it would require significant example images. 

Given the ground truth label and the teacher network's output distribution, we want the student network to not only predict the correct predicate labels but also mimic the linguistic knowledge regularized distributions. This is accomplished using a cross-entropy loss (see Eq.~\ref{objective}).
% Algorithm \ref{distillation} shows the Linguistic Knowledge distillation (LK-distillation) framework. 

One advantage of this LK distillation framework is that it takes advantage of both knowledge-based and data-driven systems. Distillation works as a regularizer to help train the data-driven system. On the other hand, since we construct the teacher network based on the student network, the knowledge regularized predictions (teacher's output) will also be improved during training as the student's output improves. Rather than using linguistic knowledge as a post-processing step, our framework enables the data-driven model to absorb the linguistic knowledge together with the ground truth labels, allowing the deep network to learn a better visual model during training rather than only having its output modified in a post-processing step.
This leads to a data-driven model (the student) that generalizes better, especially in the zero-shot scenario where we lack linguistic knowledge about a \twotup{subj}{obj} pair. While \cite{hinton,eric1,eric2} used either the student or the teacher as the final output, our experiments show that both the student and teacher in our framework have their own advantages, so we combine them to achieve the best predictive power (see section \ref{exp}).

% \begin{algorithm}
% \caption{Linguistic Knowledge distillation}\label{distillation}
% \begin{algorithmic}[1]
% \State $\mathbf{Input: }$
% \State $\quad \quad\text{Cropped images of union of objects.} $
% \State $\quad \quad \text{Linguistic knowledge:} P_d(pred|subj,obj). $

% \State $\quad \quad \text{Bounding boxes of subjects/objects}$ 
% \State $\quad \quad \text{Confidence Scores of the categories of subjects/objects.}  $ 
% \State $\quad \quad \text{Balancing parameters: } C \text{ and } \alpha.  $ 
% \State $\mathbf{repeat}$
% \State $\quad \quad \text{Sample a batch } (X,Y_{GT}).$
% \State $\quad \quad \text{Concatenate union, semantic and spatial features. }$
% \State $\quad \quad \text{Obtain student's output: } s(Y|X).$
% \State $\quad \quad \text{Construct teacher's output: } t(Y).$
% \State $\quad \quad \text{LK-distillation using Eq. \ref{objective}. }$
% \State $\mathbf{until} \quad \text{convergence}$
% \end{algorithmic}
% \end{algorithm}

\subsubsection{Linguistic Knowledge Collection}
To obtain the linguistic knowledge $P(pred|subj,obj)$, a straightforward method is to count the statistics of the training annotations, which reflect the knowledge used by an annotator in choosing an appropriate predicate to describe a visual relationship. Due to the long tail distribution of relationships, a large number of combinations never occur in the training data; however, it is not reasonable to assume the probability of unseen relationships is 0. To tackle this problem, one can apply additive smoothing to assign a very small number to all 0's \cite{add_k}; however, the smoothed unseen conditional probabilities are uniform, which is still confusing at LK distillation time. To collect more useful linguistic knowledge of the long-tail unseen relationships, we exploit text data from the Internet.

One challenge of collecting linguistic knowledge online is that the probability of finding text data that specifically describes objects and their relationships is low. This requires us to obtain the knowledge from a huge corpus that covers a very large domain of knowledge. Thus we choose the Wikipedia 2014-06-16 dump containing around 4 billion words and 450 million sentences that have been parsed to text by \cite{wiki}\footnote{The Wikipedia text file can be found on \url{http://kopiwiki.dsd.sztaki.hu/}} to extract knowledge. 

% Another challenge is that visual relationships, which are highly abstracted, may be written implicitly with a large number of variations rather than explicitly in natural language.
We utilize the scene graph parser proposed in \cite{SGParser} to parse sentences into sets of \threetup{subj}{pred}{obj} triplets, and we compute the conditional probabilities of predicates based on these triplets.
However, due to the possible mistakes of the parser, especially on text from a much wider domain than the visual relationship detection task, the linguistic knowledge obtained can be very noisy. Naive methods such as using only the linguistic knowledge to predict the predicates or multiplying the conditional probability with the data-driven model's output fail. Fortunately, since the teacher network of our LK-distillation framework is constructed from the student network that is also supervised by the labeled data, a well-trained student network can help correct the errors from the noisy external probability. 
To achieve good predictive power on the seen and unseen relationships, we obtain the linguistic knowledge from both training data and the Wikipedia text corpus by a weighted average of their conditional probabilities when we construct the teachers' network, as shown in Eq.~\ref{objective}. We conduct a two-step knowledge distillation: during the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term $C$ as shown in Eq.~\ref{objective}. 
The balancing terms are chosen by a validation set we select randomly from the training set (\eg, in VRD dataset, we select 1,000 out of 4,000 images to form the validation set) to achieve a balance between good generalization on the zero-shot and good predictive power on the entire testing set. 
% We observe that when the weight of external knowledge increases, the performance on the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 


\subsection{Semantic and Spatial Representations}
In \cite{VRD}, Lu \etal used the cropped image containing the union of two objects' bounding boxes to predict the predicate describing their relationship. While the cropped image encodes the visual appearance of both objects, it is difficult to directly model the strong semantic and spatial correlations between predicates and objects, as both semantic and spatial information is buried within the pixel values of the image. Meanwhile, the semantic and spatial representations capture similarities between visual relationships, which can generalize better to unseen relationships.

We utilize word-embedding \cite{word2vec} to represent the semantic meaning of each object by a vector. We then extract spatial features similarly to the ones in \cite{varun}:
\begin{equation}
\label{Spatial_Feature}
\left[\frac{x_{min}}{W},\frac{y_{min}}{H},\frac{x_{max}}{W},\frac{y_{max}}{H},\frac{A}{A_{img}}\right],
\end{equation}
where $W$ and $H$ are the width and height of the image, $A$ and $A_{img}$ are the areas of the object and the image, respectively. We concatenate the above features of two objects as the spatial feature (SF) for a \twotup{subj}{obj} pair. 

We predict the predicate conditioned on the semantic and spatial representations of the subject and object:
\begin{align}
\label{decompose}
P(R|I) =&P(pred|subj,obj,B_s,B_o,I)\nonumber \\
&~~ \cdot P(subj,B_s|I)P(obj,B_o|I),
\end{align}
where $subj$ and $obj$ are represented using the semantic object representation, $B_s$ and $B_o$ are the spatial features, and $I$ is the image region of the union of the two bounding boxes. 
For the BB-Union input, we use the same VGG-net \cite{VGG} in \cite{VRD} to learn the visual feature representation. 
We adopt a pre-trained word2vec vectors weighted by confidence scores of each object category for the subject and the object, then concatenate the two vectors as the semantic representation of the subject and the object.
% More details can be found in the supplementary materials.

==> 906 2/Sup.tex <==

\section{Semantic and Spatial Representations}

Spatial features have been demonstrated to be helpful in visual tasks such as object detection, image retrieval and semantic segmentation \cite{rich,o1,o2,o3,o4,o5,Ang}. For visual relationship detection task,
spatial features such as the relative location and size of two objects are informative for predicate prediction. For example, relative location is a discriminative feature for predicates ``under" and ``above" of the VRD training set shown in Figure \ref{fig:under} and \ref{fig:above}. To explicitly model the spatial location and size of an object,  we use the features from \cite{varun}:
\begin{equation}
\label{Spatial_Feature}
\left[\frac{x_{min}}{W},\frac{y_{min}}{H},\frac{x_{max}}{W},\frac{y_{max}}{H},\frac{A}{A_{img}}\right]
\end{equation}
where $W$ and $H$ are the width and height of the image, $A$ and $A_{img}$ are the areas of the object and the image, respectively. We concatenate the above features of two objects as the spatial feature (SF) for a \twotup{subj}{obj} pair. 


% \begin{figure}
% \centering     
% \subfigure[Number of \twotup{subj}{obj} Pairs vs. Number of Possible Predicates]{\label{fig:NI_Entropy}\includegraphics[width=40mm]{images/Pair.pdf}}
% \subfigure[Example to illustrate LK Distillation.]{\label{fig:example}\includegraphics[width=40mm]{images/cropped_sample}}
% \caption{(a). Most of the \twotup{subj}{obj} pairs has very a limited number of predicates that are used to describe their relationship. (b). The top-right distribution is the output of the student network; the bottom-right one is the teacher's output after penalizing the unlikely predicates given the \twotup{subj}{obj} pair.}
% \end{figure}

\begin{figure}[b]
\centering
  \includegraphics[width=70mm]{images/Pair.pdf}
  \caption{Number of \twotup{subj}{obj} Pairs vs. Number of Possible Predicates}
\label{fig:NI_Entropy}
\end{figure}

\begin{figure}[t]
\centering     
\subfigure[under]{\label{fig:under}\includegraphics[width=20mm]{images/under.eps}}
\subfigure[above]{\label{fig:above}\includegraphics[width=20mm]{images/above.eps}}
\subfigure[on]{\label{fig:on}\includegraphics[width=20mm]{images/on.eps}}
\subfigure[in]{\label{fig:in}\includegraphics[width=20mm]{images/in.eps}}
\caption{Relative location of subjects and objects for different predicates. Red box (coordinates normalized as $[0,0,1,1]$ for $[x_1,y_1,x_2,y_2]$) is the subject, blue boxes are the objects. Predicates like ``under" and ``above" are discriminative based on relative location. However, ``on" and ``in" are different to distinguish.}
\end{figure}

Given a fixed \twotup{subj}{obj} pair, only a few predicates are relevant, something which emerges by a simple analysis of linguistic descriptions of objects and their relationships. Considering that most of the \twotup{subj}{obj} pairs of the VRD training dataset have a limited number of relevant predicates.
% which indicates that given \twotup{subj}{obj} pairs, the number of plausible predicates is very limited. 
The strong correlation between a predicate and the \twotup{subj}{obj} pairs indicates that the semantic object representation  (a description of its type or class) should be informative for relationship detection, especially when the spatial features are ambiguous for different predicates. For instance, the relative bounding box locations of the subject and object \wrt predicate ``on" and ``in" as shown in \ref{fig:on} and \ref{fig:in} are similar, but given a subject of type "plate" and an object of type ``table", common sense predicts ``on" as the predicate. 
% Unlike \cite{VRD} which utilized the likelihood of \threetup{subj}{pred}{obj} combinations in their language module, our semantic representation that considers only the objects is more general.


% We predict the predicate conditioned on the semantic and spatial representations of the subject and object:
% \begin{align}
% \label{decompose}
% P(R|I) =&P(pred|subj,obj,B_s,B_o,I)\nonumber \\
% &~~\cdot P(subj,obj,B_s,B_o|I)
% \end{align}
% where $subj$ and $obj$ are represented using the semantic object representation (word2vec \cite{word2vec} is used and confidence score distribution is obtained from object detection), $B_s,B_o$ are the spatial features and $I$ is the image region of the union of the two bounding boxes.



\subsection{Evaluation of Semantic and Spatial Representations}
We evaluate the use of semantic object representations and the spatial features without LK distillation. We compare our method with three methods in \cite{VRD} and \cite{VisualPhrase}: ``Visual Phrases" denotes the method that trains deformable parts models for each relationships; ``Joint CNN" denotes the method trains a 270-way CNN model to predict the subject, object and predicate together. ``VRD - V only" denotes the method proposed in \cite{VRD} that uses VGG-net to extract features for the BB-Union of two bounding boxes and then feeds the features into a learned linear model to predict the predicate. Besides the existing methods, we also compare our method with a baseline that uses the same VGG-net as \cite{VRD} and BB-Union of boxes but with end-to-end training  (denoted as ``Baseline: U"). To test the use of our semantic and spatial features, we test different combinations, shown in Table \ref{P:visual} and Table \ref{P:visualZero}. 

\begin{table}[t]
\centering
\caption{Predicate Detection: Different Visual Features. ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``one-hot" and ``word2vec" are two semantic representations.}
\label{P:visual}\vskip 3pt
% \resizebox{\textwidth}{!}
% \footnotesize
\scriptsize
%\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
                    & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.},                                & R@100,                 & R@50,                                  \\
& k=1                                       & k=70                   & k=70                   \\\midrule
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -          \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -          \\
VRD - V only  \cite{VRD}        & 7.11             & 37.20           & 28.36          \\
% Linguistic Cues       & -          & -         & -           & -          \\
\midrule
Baseline: U                 & 34.82          & 83.15       & 70.02      \\
U + one-hot        & 36.42           & 84.66       & 71.07      \\
U + word2vec      & 37.15          & 83.78       & 70.75      \\
U + SF            & 36.33           & 83.68       & 69.87           \\
U + one-hot + SF   & 38.87           & 84.34       &71.79      \\
U + word2vec + SF & \textbf{41.33}          & \textbf{84.89}       &  \textbf{72.29}      \\ \bottomrule
\end{tabular}
\end{table}

Table \ref{P:visual} reveals that end-to-end training (our ``Baseline: U ") with soft-max prediction outperforms the feature+linear model method (``VRD - V only"), highlighting the importance of fine-tuning. In addition, adding semantic or spatial features individually improves the predictive power of the data-driven model. The combination of BB-Union, semantic and spatial features yields the best performance. 

We report the performance of different methods on zero-shot predicate prediction task in Table \ref{P:visualZero}. Our end-to-end CNN model using BB-Union, semantic and spatial features outperforms \cite{VRD} by a large margin in the zero-shot setting. Among the three sets of features, the spatial feature generalizes best, the one-hot feature the worst, the word2vec feature in between. We believe that this is because some \twotup{subj}{obj} pairs in the zero-shot setting never occur in the training set, and the one-hot feature is too specific to generalize from the seen pairs to the unseen pairs. 
The word2vec features generalize better because the formulation of the vector space already takes the semantic similarity of different objects into consideration. 
% Since the zero-shot setting is only on semantic level, 
Spatial features that capture low level information of bounding boxes generalize the best.

\begin{table}[]
\centering
\caption{Predicate Detection: Different Visual Features - Zero Shot. We use the same notations as in Table \ref{P:visual}.}\vskip 3pt
\label{P:visualZero}
% \footnotesize
\scriptsize
%\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
                      & R@100/50,                                 & R@100,                 & R@50,                                  \\
& k=1                                     & k=70                   & k=70                   \\\midrule
VRD - V only \cite{VRD}               & 3.52      & 32.34           & 23.95          \\ 
% Linguistic Cues       & -          & -         & -           & -          \\
\midrule
Baseline: U                     & 12.75     & 69.42       & 47.84      \\
U + one-hot            & 11.86     & 69.46       & 47.22      \\
U + word2vec           & 13.44     & \textbf{69.77}       & \textbf{49.01}      \\
U + SF                & \textbf{14.33}     & 69.01       & 48.32      \\
U + one-hot + SF        & 12.98     & 69.35       & 48.79      \\
U + word2vec + SF       & 14.13     & 69.41       & 48.13      \\ \bottomrule
\end{tabular}
\end{table}

\subsection{When do Spatial Features Help?}
To show the role of spatial features in visual relationship detection task, We observe from Figure \ref{fig:NI_Entropy} that most of the \twotup{subj}{obj} pairs have low entropy in their predicate distribution, which implies a strong correlation between a predicate and \twotup{subj}{obj} pairs. It is interesting to understand why adding the spatial features outperforms a model that already knows which objects it is analyzing. We choose the method ``U + word2vec + SF" and ``U + word2vec" to evaluate when spatial features help. Our hypothesise is that SF helps when \twotup{subj}{obj} is not very deterministic. 
% One measurement to model the uncertainty of the predicate given \twotup{subj}{obj} is the entropy of predicate distribution. 
We plot the ``R@100/50, k=1" improvement of ``U + word2vec + SF" over ``U + word2vec" vs. the entropy of $P(pred|subj,obj)$ in Figure \ref{fig:Entropy}.

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\linewidth]{images/Entropy.eps}
%   \caption{R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$}
% \label{fig:Entropy}
% \end{figure}

% \begin{figure}
% \centering     
% \subfigure[ ]{\label{fig:Entropy}\includegraphics[width=40mm]{images/Entropy.eps}}
% \subfigure[ ]{\label{fig:im}\includegraphics[width=40mm]{images/Improve_number_histo.pdf}}
% \caption{(a). R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$ (b). Recall@100 Improvement with LK-distillation vs. the number of training \twotup{subj}{obj} pairs.}
% \end{figure}

\begin{figure}[t]
\centering
  \includegraphics[width=70mm]{images/Entropy.eps}
  \caption{R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$}
\label{fig:Entropy}
\end{figure}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\linewidth]{images/Improve_number_histo.pdf}
%   \caption{Recall@100 Improvement with LK-distillation vs. the number of training \twotup{subj}{obj} pairs.}
% \label{fig:im}
% \end{figure}



We notice that when the entropy is small (\twotup{subj}{obj} is deterministic), most of the relationships with those \twotup{subj}{obj} pairs do not benefit from adding spatial features. However, when the entropy is large (1-1.5), adding spatial features improves predictive power for those relationships. 



% \subsubsection{Knowledge Transfer with Linguistic Knowledge Distillation}

% One application of our LK distillation framework is that if we can obtain reasonable good linguistic knowledge, we can use very limited training data to obtain 

% \begin{table}[]
% \centering
% \caption{Knowledge Transfer: Train on VRD dataset with the linguistic knowledge from VG; test on VG dataset. We use the same notations as in Table \ref{VG}.}
% \label{transfer}\vskip 3pt
% % \footnotesize
% \scriptsize
% \setlength\tabcolsep{5pt}
% \begin{tabular}{@{}lccc@{}}
% \toprule
%                                  & R@100/50,                               & R@100,                 & R@50,                                  \\
% & k=1                                 & k=70                   & k=70                   \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Train and test on VG}} \\
% U+W+SF               & 40.62    & 86.65    & 83.91       \\
% U+W+SF+L: S         & 49.88    & 91.25    & 88.14      \\
% U+W+SF+L: T         & 55.02    & 94.92    & 91.47       \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 2: Train on VRD with LK from VG; test on VG}} \\
% U+W+SF               & 32.08    & 78.43    & 72.46       \\
% U+W+SF+L: S         & 45.89    & 91.32    & 82.73      \\
% U+W+SF+L: T         & 52.26    & 94.06    & 90.53       \\\midrule

% \end{tabular}
% \end{table}

\section{Linguistic Knowledge Distillation with More Training Images} 
Another interesting finding is that LK-distillation offers higher performance improvement for the relationships that  have few training instances, which is also reported in \cite{eric2} (details can be found in the supplementary materials). This observation supports our motivation that knowledge helps the long-tail relationships most.

A natural question is: can we just collect more data and obtain significant improvement in predictive power and generalization? To answer this question, we utilize the recently proposed Visual Genome dataset \cite{VG} to augment the training data of VRD. By selecting the relationship instances and have predicates and objects in the categories of VRD dataset from images that are not in VRD set from Visual Genome set, we obtain around 130K more training instances, enlarging the original VRD training set by 5$\times$. To make the zero-shot testing set of VRD remain unseen, we ensure that the relationships in the zero-shot set are excluded from the augmented training data. We conduct similar experiments with the augmented dataset and distill the same linguistic knowledge extracted from VRD dataset. The results are shown in the Part 2 of 
Table 1, 2 and 3 in the main paper. 
We observe that training with more data leads to only marginal performance improvement of almost all baselines and proposed methods. However, for all experimental settings, with more data, our LK distillation framework still brings significant improvements, and the combination of the teacher and student networks still yields the best performance. The experiments imply that simply adding more training images does not help much. One reason we observe is that the distribution of relationships in the newly added images are still long-tail (although the Visual Genome dataset is much larger than VRD), the data-driven model still does not get enough training data. Another reason is that since we still use the linguistic knowledge extracted from VRD set, the strong linguistic prior dominates the predictions so that we observe the performance of teacher networks are very similar with/without the newly added images from Visual Genome dataset. Both reasons imply that we may need to extract the linguistic knowledge from a larger domain that contains more unseen relationships.

% \begin{table}[]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3.5pt} 
% \caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them. \textbf{Part 1} uses the training images in VRD dataset and \textbf{Part 2} uses the training images in VRD \cite{VRD} and all images of Visual Genome (VG) \cite{VG} dataset.}
% \label{P_VRD_1}
% \begin{tabular}{@{}lccc|ccc@{}}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
% \multicolumn{1}{@{}l}{ } & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
% \multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}} &&&& \\
% Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
% Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

% VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
% VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

% Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
% Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
% U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
% U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
% U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
% U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
% U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
% U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
% U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
% U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
% U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
% U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\\midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
% \bottomrule
% \end{tabular}
% \end{table}




% \begin{table*}[t]
% \centering
% \caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD_1}.}\vskip 3pt
% \label{Detection_1}
% % \footnotesize
% \scriptsize
% \setlength\tabcolsep{3.5pt}
% \begin{tabular}{@{}lcccccc|cccccc@{}}
% \toprule
% & \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% % \textbf{Part 1: VRD only} 
% & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
% & k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}}&&&&&&&&&&\\
% VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
% Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
% U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
% U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
% U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\

% \end{tabular}
% \end{table*}



% \begin{table*}[t]
% \centering
% % \footnotesize
% \scriptsize
% \caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD_1}.}\vskip 3pt
% \setlength\tabcolsep{3.8pt}
% \label{Detection_Zero_1}
% \begin{tabular}{@{}lcccccc|cccccc@{}}
% \toprule
%                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
%                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
%                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}}&&&&&&&&&&\\

% VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
% Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
% U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
% U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\


% \end{tabular}
% \end{table*}



==> 906 2/exp_back.tex <==
\section{Experiments}\label{exp}
\subsection{Dataset}
We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
%   \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
%   \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \end{itemize}


\subsection{Implementation Details}
We use VGG-net \cite{VGG} to learn the visual representations of the BB-Union of two objects. For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, we use a pre-trained word2vec model to project the subjects and objects into vector space, and the final representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\subsection{Evaluation Metric}
We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in VRD is not exhaustive \cite{VRD}).
The standard Recall@n metric ranks all predictions for an image and choose the top n predictions. However, \cite{VRD} evaluated only the top prediction for each pair, and rank the predictions for all pairs in a image, then ranked these select the top n to report the Recall@n. By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
Considering multiple predicates can correctly describe the same object pair, (e.g. when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
we believe that a good predicted probability distribution of a predicate that captures the semantic similarity between plausible predicates should has large probability of plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalizes correct predictions because of the annotator's preference or random choice from several plausible predicates. 
% Since there are multiple pairs of objects in an image, and each pair has 70 predictions with different confidence scores, 

We treat the number of chosen predictions per pair (k) as a hyper-parameter, and report R@n for two different $k$'s: 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}



\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our proposed method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate our method given ground truth object detection results, which is the predicate prediction tasks in \cite{VRD}. Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. Since \cite{UIUC} does not report the results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}.

Table \ref{P_VRD} show the evaluation of linguistic knowledge distillation with different set of features in our deep neural networks. In addition to the data-driven baseline, we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". ``Visual Phrases" denotes the method that trains deformable parts models for each relationships \cite{VisualPhrase}; ``Joint CNN" denotes the method trains a 270-way CNN model to predict the subject, object and predicate together. The visual model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". In both tables, S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline that uses the same visual representation (BB-Union) as \cite{VRD} and the ``VRD-V only" model, the huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 31.62\% (ours)) reveals that the end-to-end training with soft-max prediction outperforms the extracting feature from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding semantic representation and spatial features improves the predictive power and generalization of the data-driven model. More analysis on using different combination of features can be found in the supplementary materials.



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{} &&&& \\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\
% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships in training data]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Unseen relationships in training data]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of Predicate Detection: Different Methods. ``Data-driven" denotes the Baseline: U; ``LK only" denotes the Baseline: L only; ``Full model student" denotes the U+W+SF+LK: S; ``Full model teacher" denotes the U+W+SF+LK: T.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\

VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\

\bottomrule


\end{tabular}
\end{table*}


To demonstrate the effectiveness of our LK-distillation framework, we compare the results of using different combinations of features with/without using LK-distillation. In Part 1 of table \ref{P_VRD}, for fair comparison with the existing methods, we train and test our model on VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the data-driven baseline all of the state-of-the-art methods (\cite{VisualPhrase}, \cite{Rcnn} and \cite{VRD}) by a large margin (e.g. 51.34\%  vs. 47.87\% \cite{VRD} for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without even looking at the images leads to very pool performance on the zero-shot set of VRD, which implies the poor generalization of ``Baseline: L only" method and addresses the need of combining both data-driven and knowledge-based method as the LK-distillation framework we propose.

To show the benefit of LK-distillation, we observe a consistent trend that for all feature settings, the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models by a large margin, (e.g. R@100/50, k=1 is improved from 33.48\% to 40.95\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in training data; the other is that although the linguistic priors are powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far away from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels be equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin (e.g. 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework have their own advantages. The best predictive power is achieved when we combine them together: we use teacher's network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. Setting ``U+W+SF+LK: T+S" achieves the best performance. One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. Visualizations of different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we follow \cite{VRD} to use a R-CNN based detector \cite{Rcnn} for object detection tasks. Given the confidence scores of each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution of each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with methods in \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report the recall. In addition, we report the standard recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Part 1 of Table \ref{Detection} and \ref{Detection_Zero}. 

We observe that our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} by a large margin on both entire testing set and the zero-shot setting. The observations about student and teacher networks are consistent with the ones in predicate prediction evaluation. On the other hand, when comparing the results of predicate and relationship prediction, the large performance margin (53.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental task such as object detection.

\subsection{Evaluation on Visual Genome Dataset}

To show our generic framework works on different data distribution, we evaluate our method on Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct similar evaluation on this much larger dataset (99,864 relationship instances for training and  19,754 for testing. In the testing set, 2,056 relationships instance are never seen in the training data.) using the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar results as our experiments on VRD dataset that the LK distillation method manages to regularize the learning process of the deep model and improve its predictive power and generalization. We also conduct another experiment that we use images in Visual Genome dataset to augment the training set of VRD and still test on VRD dataset. When the R@100/50 k=1 of pure data-driven model for predicate detection is improved from 31.62\% to 33.67\% due to a larger training set, our LK-distillation boosts the recall to 53.38\%, which reveals that incorporating additional knowledge brings more benefits than collecting more data. More details can be found in the supplementary materials. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset: We use the same notations as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 36.83    & 83.05    & 81.38    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.62    & 86.65    & 83.91    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits from extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
For those unseen long-tail relationships in VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results using our linguistic knowledge distillation framework, then testing on VRD dataset with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, an interesting finding is that, although the external knowledge can be very noisy (Wikipedia) or has a different distribution when compared with the VRD dataset (Visual Genome), the performance of teacher network using external knowledge is much better than the one restricted in the VRD training dataset (Part 1). 
That finding suggests that by properly distilling the external knowledge, our framework may manage to obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 

To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. \textbf{Part 1} uses the LK from VRD dataset; \textbf{Part 2} uses the LK from VG dataset; \textbf{Part 3} uses the LK from both VRD and VG dataset. \textbf{Part 4} uses the LK from parsing Wikipedia text; \textbf{Part 5} uses the LK from from both VRD dataset and Wikipedia. We use the same notations as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\textbf{Part 1 LK: VRD}  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S         & 45.50    & 85.67    & 74.98    & 15.53   & 71.15    & 52.21  \\
U+W+SF+L: T         & 53.03    & 88.43    & 81.78    & 8.30    & 40.03    & 31.31   \\\midrule
\textbf{Part 2 LK: VG} & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 15.31   & 69.29    & 48.59   \\
U+W+SF+L: T         & 51.00    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{\textbf{Part 3 LK: VRD+VG}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 16.88    & 74.09   & 54.29   \\
U+W+SF+L: T         & \textbf{53.67}    & \textbf{90.13}    & \textbf{83.63}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 4 LK: Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 5 LK: VRD+Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 47.64   & 88.21   & 77.79    & \textbf{18.17}    & \textbf{75.62}    & \textbf{56.45}   \\
U+W+SF+L: T         & 52.14    & 88.23   & 81.78    & 8.95     & 39.24   & 30.61  \\\bottomrule
\end{tabular}
\end{table}


We observe that by properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (e.g. \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.







==> 906 2/exp_back_0309.tex <==
\section{Experiments}\label{exp}
% We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
We evaluate our LK-distillation method on the Visual Relationship Detection \cite{VRD} and Visual Genome \cite{VG} datasets. There are three evaluation tasks:
% 1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
% 2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
% 3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\begin{itemize}
\itemsep -1pt
  \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
  \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
  \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\end{itemize}

Both datasets have a zero-shot testing set that contains relationships that never occur in the training data. We also evaluate our approaches on the zero-shot sets to demonstrate the improvement on generalization by linguistic knowledge distillation.

\textbf{Implementation Details.} We use VGG-net \cite{VGG} to learn the visual representations of the BB-Union of two objects. For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. 
% For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, 
We use a pre-trained word2vec model to project the subjects and objects into vector space, and the final semantic representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\textbf{{Evaluation Metric.}} We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in the datasets are not exhaustive).
For two detected objects, there can be multiple predicate predictions with different confident scores. The standard Recall@n metric ranks all predictions for all detected object pairs in an image and chooses the top n predictions to compute the recall. However, in contrast of computing recall based on all predictions, \cite{VRD} evaluated only the prediction with highest confident score for each object pair. 
By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
However, considering the fact that multiple predicates can correctly describe the same object pair, (e.g., when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
we believe that a good predicted probability distribution of a predicate that captures the semantic similarity between plausible predicates should have large probability for plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalize correct predictions because of the annotator's preference or random choice amongst several plausible predicates. 
% Since there are multiple pairs of objects in an image, and each pair has 70 predictions with different confidence scores, 

We treat the number of chosen predictions per object pair (k) as a hyper-parameter, and report R@n for different $k$'s to compare with other state-of-the-art methods \cite{VRD,UIUC,VisualPhrase}. Since the number of predicates is 70, $k=70$ is equivalent to getting every predictions of two detected objects into evaluation. 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
% 1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
% 2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}

\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate it given ground truth object detection results, which is the predicate prediction task in \cite{VRD}. 
% Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. 
Since \cite{UIUC} does not report results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}.

Table \ref{P_VRD} shows the evaluation of linguistic knowledge distillation with different sets of features in our deep neural networks. In addition to the data-driven baseline ``Baseline: U only", we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". The "Visual Phrases" method \cite{VisualPhrase} trains deformable parts models for each relationships ; ``Joint CNN" \cite{Rcnn} trains a 270-way CNN model to predict the subject, object and predicate together. The visual model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline that uses the same visual representation (BB-Union) as \cite{VRD} and the ``VRD-V only" model, the huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 31.62\% (ours)) reveals that the end-to-end training with soft-max prediction outperforms extracting features from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding the semantic representation and the spatial features improves the predictive power and generalization of the data-driven model. \footnote{More analysis on using different combinations of features can be found in the supplementary materials.}



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{} &&&& \\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20\tablefootnote{The results of Recall when k=70 are not reported in \cite{VRD}. To show the improvement of our method with different k's we calculate those recall values using their code. The same for Table \ref{Detection} and \ref{Detection_Zero}.}           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\
% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships in training data]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Unseen relationships in training data]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of predicate detection results: ``Data-driven" denotes the baseline using BB-Union; ``LK only" denotes the baseline using only the linguistic knowledge without looking at the image; ``Full model student" denotes the student network with U+W+SF features; ``Full model teacher" denotes the teacher network with U+W+SF features.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\

VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\

\bottomrule


\end{tabular}
\end{table*}

To demonstrate the effectiveness of our LK-distillation framework, we compare the results of using different combinations of features with/without using LK-distillation. In table \ref{P_VRD}, for fair comparison with existing methods, we train and test our model on the VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the state-of-the-art method \cite{VRD} by a large margin (e.g., 51.34\%  vs. 47.87\% for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without even looking at the images leads to very pool performance on the zero-shot set of VRD, which explains the poor generalization of ``Baseline: L only" method and addresses the need for combining both data-driven and knowledge-based methods as the LK-distillation framework we propose does.

To show the benefit of LK-distillation, we observe a consistent trend that for all feature settings, the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models significantly (e.g., R@100/50, k=1 is improved from 33.48\% to 40.95\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in the training data; the other is that although the linguistic prior is powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on the zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin (e.g., 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework have their own advantages. The best predictive power is achieved when we combine them together: we use the teacher network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. The setting ``U+W+SF+LK: T+S" achieves the best performance. 
% One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. 
Visualizations of the different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we follow \cite{VRD} to use an R-CNN based detector \cite{Rcnn} for object detection tasks. Given the confidence scores of each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution for each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report the recall. In addition, we report the standard recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Tables \ref{Detection} and \ref{Detection_Zero}. 

Our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} significantly on both entire testing set and zero-shot setting. The observation about student and teacher networks are consistent with predicate prediction evaluation. Additionally, when comparing the results of predicate and relationship prediction, the large performance gain (53.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental object detection task.

\subsection{Evaluation on Visual Genome Dataset}

We also evaluate our method on the Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations, on the predicate detection task. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct similar evaluation on the dataset (99,864 relationship instances in training and 19,754 in testing. In the testing set, 2,056 relationships instance are never seen in the training data). We use the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar behavior as our experiments on the VRD dataset--LK distillation manages to regularize the deep model and improve its generalization. We conduct another experiment in which images from Visual Genome dataset augment the training set of VRD and evaluate on the VRD test set\footnote{Details can be found in the supplementary materials.}. While the R@100/50 k=1 measure of the purely data-driven model for predicate detection improves from 31.62\% to 33.67\% due to the increased training size, our LK-distillation boosts recall to 53.38\%, which reveals that incorporating additional knowledge is more beneficial than collecting more data. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset. Notations are the same as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 36.83    & 83.05    & 81.38    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.62    & 86.65    & 83.91    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits of extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
% However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
However, training annotations only represent a small portion of all possible relationships and do not necessarily represent the real world distribution, which is essentially long tail.
For those unseen long-tail relationships in the VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results on the VRD test set using our linguistic knowledge distillation framework with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, interestingly, although the external knowledge can be very noisy (Wikipedia) or have a different distribution when compared with the VRD dataset (Visual Genome), the performance of the teacher network using such external knowledge is much better than that restricted to the VRD training dataset (Part 1). 
This finding suggests that by properly distilling the external knowledge, our framework can obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 
% To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
% After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
% The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
% We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. We observe that by distilling external knowledge with the internal one, we improve the generalization significantly (e.g., LK from Wikipedia boosts the recall to 18.17\% on the zero-shot set) while maintaining good predictive power on the entire test set.

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. \textbf{Part 1} uses the LK from VRD dataset; \textbf{Part 2} uses the LK from VG dataset; \textbf{Part 3} uses the LK from both VRD and VG dataset. \textbf{Part 4} uses the LK from parsing Wikipedia text; \textbf{Part 5} uses the LK from from both VRD dataset and Wikipedia. Notations are the same as as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\textbf{Part 1 LK: VRD}  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S         & 45.50    & 85.67    & 74.98    & 15.53   & 71.15    & 52.21  \\
U+W+SF+L: T         & 53.03    & 88.43    & 81.78    & 8.30    & 40.03    & 31.31   \\\midrule
\textbf{Part 2 LK: VG} & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 15.31   & 69.29    & 48.59   \\
U+W+SF+L: T         & 51.00    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{\textbf{Part 3 LK: VRD+VG}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 16.88    & 74.09   & 54.29   \\
U+W+SF+L: T         & \textbf{53.67}    & \textbf{90.13}    & \textbf{83.63}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 4 LK: Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 5 LK: VRD+Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 47.64   & 88.21   & 77.79    & \textbf{18.17}    & \textbf{75.62}    & \textbf{56.45}   \\
U+W+SF+L: T         & 52.14    & 88.23   & 81.78    & 8.95     & 39.24   & 30.61  \\\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
  \includegraphics[width=60mm]{images/I_N}
  \caption{Performance with varying sizes of training examples. ``Our Method" denotes the student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text. ``VRD-Full" is the full model in \cite{VRD}.}
\label{fig:im}
\end{figure}

We show the performance comparisons between our student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text (denoted as ``Our Method") and the full model in \cite{VRD} (denoted as ``VRD-Full") in Figure \ref{fig:im}. We observe that our method significantly outperforms the existing method, especially in the zero-shot (number of training instance is 0) and the few-shot setting (number of training instance is small, e.g., $<10$), which reveals that by distilling linguistic knowledge into a deep model, we can dramatically improve the generalization of our data-driven model, which is hard to achieve by only training it on limited labeled images.



% By properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
% By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (e.g. \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.











==> 906 2/exp_back_0315.tex <==
\section{Experiments}\label{exp}
% We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
We evaluate our method on the Visual Relationship Detection \cite{VRD} and Visual Genome \cite{VG} datasets. There are three evaluation tasks:
% 1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
% 2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
% 3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\begin{itemize}
\itemsep -1pt
  \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
  \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
  \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\end{itemize}

Both datasets have a zero-shot testing set that contains relationships that never occur in the training data. We also evaluate on the zero-shot sets to demonstrate the generalization improvements brought by linguistic knowledge distillation.

\textbf{Implementation Details.} We use VGG-16 \cite{VGG} to learn the visual representations of the BB-Union of two objects. 
% For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. 
% For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, 
We use a pre-trained word2vec model to project the subjects and objects into vector space, and the final semantic representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\textbf{{Evaluation Metric.}} We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in the datasets are not exhaustive).
For two detected objects, there can be multiple predicate predictions with different confident scores. The standard Recall@n metric ranks all predictions for all detected object pairs in an image and chooses the top n predictions to compute the recall. However, instead of computing recall based on all predictions, \cite{VRD} evaluated only the prediction with highest confident score for each object pair. 
By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
However, multiple predicates can correctly describe the same object pair, (\eg, when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
so we believe that a good predicted probability distribution should have large probability for all plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalize correct predictions because of the annotator's preference or random choice amongst several plausible predicates. 
Thus, we treat the number of chosen predictions per object pair (k) as a hyper-parameter, and report R@n for different $k$'s to compare with other state-of-the-art methods \cite{VRD,UIUC,VisualPhrase}. Since the number of predicates is 70, $k=70$ is equivalent to getting every predictions of two detected objects into evaluation. 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
% 1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
% 2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}

\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate it given ground truth object detection results, which is the predicate prediction task in \cite{VRD}. 
% Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. 
Since \cite{UIUC} does not report results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}. 

Part 1 of Table \ref{P_VRD} shows the evaluation of linguistic knowledge distillation with different sets of features in our deep neural networks. In addition to the data-driven baseline ``Baseline: U only", we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". The "Visual Phrases" method \cite{VisualPhrase} trains deformable parts models for each relationship; ``Joint CNN" \cite{Rcnn} trains a 270-way CNN model to predict the subject, object and predicate together. The visual only model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline, which uses the same visual representation (BB-Union) as \cite{VRD}, and the ``VRD-V only" model, our huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 34.82\%) reveals that the end-to-end training with soft-max prediction outperforms extracting features from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding the semantic representation and the spatial features improves the predictive power and generalization of the data-driven model. \footnote{More analysis on using different combinations of features can be found in the supplementary materials.}



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them. Part 1 uses the training images in VRD dataset; Part 2 uses the training images in VRD \cite{VRD} and all images of Visual Genome (VG) \cite{VG} dataset.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20
\tablefootnote{The results of Recall when k=70 are not reported in \cite{VRD}. To show the improvement of our method with different k's we calculate those recall values using their code. The same for Table \ref{Detection} and \ref{Detection_Zero}.}          
& 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 34.82     & 83.15       & 70.02    & 12.75     & 69.42       & 47.84   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 37.15     & 83.78       & 70.75   & 13.44     & 69.77       & 49.01    \\
U+W+L:S               & 42.98     & 84.94       & 71.83  & 13.89       & 72.53       & 51.37     \\
U+W+L:T               & 52.96     & 88.98       & 83.26   & 7.81          & 40.15      & 32.62   \\\hdashline
U+SF                 &36.33           & 83.68       & 69.87  & 14.33     & 69.01       & 48.32    \\
U+SF+L:S                       & 41.06     & 84.81       & 71.27    & 15.14          & 72.72       & 51.62  \\
U+SF+L:T               & 51.67     & 87.71       & 83.84     & 8.05          & 41.51       & 32.77    \\ \hdashline
U+W+SF                   & 41.33     & 84.89       & 72.29  & 14.13         & 69.41       & 48.13    \\
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & \textbf{16.98}       & \textbf{74.65}       & \textbf{54.20}    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81    \\
U+W+SF+L: T+S    & \textbf{55.16}     & \textbf{94.65}       & \textbf{85.64}    & -          & -       & -  \\
\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}
                                              & & &  &                      \\
Baseline: U                                           & 36.97     & 84.49  & 70.19   & 13.31     & 70.56  & 50.34     \\
U+W+SF                     & 42.08     & 85.89       & 72.83   & 14.51          & 70.79       & 50.64     \\
U+W+SF+L: S             & 48.61      & 87.15       & 75.45    & 17.16          & 75.26       & 55.41     \\
U+W+SF+L: T             & 54.61     & 90.09       & 82.97       & 9.23          & 43.21       & 33.40  \\
U+W+SF+L: T+S               & 55.67     &95.19      & 86.14    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Zero-shot Relationships]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of predicate detection results: ``Data-driven" denotes the baseline using BB-Union; ``LK only" denotes the baseline using only the linguistic knowledge without looking at the image; ``Full model student" denotes the student network with U+W+SF features; ``Full model teacher" denotes the teacher network with U+W+SF features.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 0.07             & 0.04           & -    & - & - & -   & -& -& -& -& -   \\
Joint CNN  \cite{Rcnn}           & 0.09             & 0.07           & -    & - & - & - & 0.09    & 0.07 & - & -& -    & -      \\
% VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & -                      & -       & -                      & -               &14.70                  & 13.86                  & -                      & -            & -                    & -          \\
VRD - V only  \cite{VRD}           & 2.61             & 2.24           & -    & - & - & - & 1.85    & 1.58 & - & -& -    & -      \\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \hdashline
U+W+SF+L: S      & 19.98 & 19.15 & 25.16 & 22.95 & 25.54	& 22.59 & 17.69 & 16.57 & 27.98 & 19.92 &28.94	&20.12\\
U+W+SF+L: T      & 22.97 & 22.06 & 29.14 & 25.96 &29.09	&25.86 & 19.81 & 18.67 & 29.36 & 21.89 &31.06	&21.96\\
U+W+SF+L: T+S  & \textbf{23.47} & \textbf{22.34} & \textbf{29.76} & \textbf{26.47} &\bf29.43	&\bf26.32 & \textbf{20.25} & \textbf{19.01} & \textbf{29.89} & \textbf{22.56} &\bf 31.89	&\bf22.68\\

\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 20.32 & 19.96 & 25.71 & 23.34 & 25.97	& 22.83 & 18.32 & 16.98 & 28.24 & 20.15 &29.85	&21.88\\
U+W+SF+L: T      & 23.32 & 22.56 & 29.89 & 26.34 &29.92	&26.15 & 20.04 & 18.91 & 29.95 & 22.42 &31.74	&22.64\\
U+W+SF+L: T+S     & 23.96 & 22.84 & 30.13 & 26.73 &30.01	&26.58 & 20.56 & 19.38 & 30.45 & 22.84 &32.56	&23.18\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&&&&&&&\\

% VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & -                     & -    & -                      & -                  & 3.52                  & 3.13                  & -                      & -      & -                     & -                \\
VRD - V only  \cite{VRD}           & 1.12             & 0.95           & -    & - & - & - & 0.78    & 0.67 & - & -& -    & -      \\
VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\hdashline
U+W+SF+L: S   & \textbf{10.89} & \textbf{10.44} & \textbf{17.24} & \textbf{13.01} &\bf 17.24	&\bf 12.96 & \textbf{9.14} & \textbf{8.89} & \textbf{16.15} & \textbf{12.31} &\bf 15.89	&\bf 12.02\\ 	
U+W+SF+L: T      & 6.71 & 6.54 & 11.27 & 9.45 &9.84	&7.86 & 6.44 & 6.07 & 9.71 & 7.82 &10.21	&8.75\\
\midrule
   
\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 11.23 & 10.87 & 17.89 & 13.53 & 17.88	& 13.41 & 9.75 & 9.41 & 16.81 & 12.72 &16.37	&12.29\\
U+W+SF+L: T      & 7.03 & 6.94 & 11.85 & 9.88 &10.12	&8.97 & 6.89 & 6.56 & 10.34 & 8.23 &10.53	&9.03\\

\bottomrule


\end{tabular}
\end{table*}

To demonstrate the effectiveness of LK-distillation, we compare the results of using different combinations of features with/without using LK-distillation. In Part 1 of Table \ref{P_VRD}, for fair comparison with existing methods, we train and test our model on only the VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the state-of-the-art method \cite{VRD} by a large margin (\eg, 51.34\%  vs. 47.87\% for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without looking at the images leads to very poor performance on the zero-shot set of VRD, which explains the poor generalization of ``Baseline: L only" method and addresses the need for combining both data-driven and knowledge-based methods as the LK-distillation framework we propose does.

The benefit  of LK distillation is visible across all feature settings: the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models significantly (\eg, R@100/50, k=1 is improved from 37.15\% to 42.98\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in the training data; the other is that although the linguistic prior is powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on the zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin.
% (\eg, 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework are used, since they each have their own advantages. The best predictive power is achieved when we combine them together: we use the teacher network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. The setting ``U+W+SF+LK: T+S" achieves the best performance. 
% One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. 
Visualizations of the different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we train a Fast R-CNN detector \cite{fastRCNN} for object detection tasks. Given the confidence scores of detected each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution for each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report recall. In addition, we report the full recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Part 1 of Tables \ref{Detection} and \ref{Detection_Zero}. Our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} significantly on both entire testing set and zero-shot setting. The observations about student and teacher networks are consistent with predicate prediction evaluation. 
% Additionally, when comparing the results of predicate and relationship prediction, the large performance gain (5.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental object detection task.

\subsection{Evaluation on Visual Genome Dataset}

We also evaluate our method on the Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations, on the predicate detection task. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct a similar evaluation on the dataset (99,864 relationship instances in training and 19,754 in testing; In the testing set, 2,056 relationships instance are never seen in the training data). We use the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar behavior as our experiments on the VRD dataset---LK distillation manages to regularize the deep model and improve its generalization. We conduct another experiment in which images from Visual Genome dataset augment the training set of VRD and evaluate on the VRD test set. From the Part 2 of Tables \ref{P_VRD}, \ref{Detection} and \ref{Detection_Zero}, we observe that training with more data leads to only marginal performance improvement of almost all baselines and proposed methods. However, for all experimental settings, with more data, our LK distillation framework still brings significant improvements, and the combination of the teacher and student networks still yields the best performance, which reveals that incorporating additional knowledge is more beneficial than collecting more data\footnote{Details can be found in the supplementary materials.}. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset. Notations are the same as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 37.81    & 82.05    & 81.41    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.92    & 86.81    & 84.92    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits of extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
% However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
However, training annotations only represent a small portion of all possible relationships and do not necessarily represent the real world distribution, which has a long tail.
For those unseen long-tail relationships in the VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results on the VRD test set using our linguistic knowledge distillation framework with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, interestingly, although the external knowledge can be very noisy (Wikipedia) or have a different distribution when compared with the VRD dataset (Visual Genome), the performance of the teacher network using such external knowledge is much better than that restricted to the VRD training dataset (Part 1). 
This finding suggests that by properly distilling the external knowledge, our framework can obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 
% To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
% After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
% The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
% We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. We observe that by distilling external knowledge with the internal one, we improve the generalization significantly (\eg, LK from Wikipedia boosts the recall to 19.17\% on the zero-shot set) while maintaining good predictive power on the entire test set.

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. Part 1 uses the LK from VRD dataset; Part 2 uses the LK from VG dataset; Part 3 uses the LK from both VRD and VG dataset. Part 4 uses the LK from parsing Wikipedia text; Part 5 uses the LK from from both VRD dataset and Wikipedia. Notations are the same as as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
Part 1 LK: VRD  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & 16.98       & 74.65       & 54.20    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81     \\\midrule
Part 2 LK: VG & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 16.88   & 72.29    & 52.51   \\
U+W+SF+L: T         & 51.54    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{Part 3 LK: VRD+VG} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 17.21    & 74.89   & 54.65   \\
U+W+SF+L: T         & \textbf{54.82}    & \textbf{90.63}    & \textbf{83.97}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{Part 4 LK: Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{Part 5 LK: VRD+Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.94   & 87.11   & 77.79    & \textbf{19.17}    & \textbf{76.42}    & \textbf{56.81}   \\
U+W+SF+L: T         & 54.06    & 88.93   & 81.78    & 9.65     & 42.24   & 34.61  \\\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
  \includegraphics[width=60mm]{images/I_N}
  \caption{Performance with varying sizes of training examples. ``Our Method" denotes the student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text. ``VRD-Full" is the full model in \cite{VRD}.}
\label{fig:im}
\end{figure}

We show performance comparisons between our student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text (denoted as ``Our Method") and the full model in \cite{VRD} (denoted as ``VRD-Full") in Figure \ref{fig:im}. We observe that our method significantly outperforms the existing method, especially for the zero-shot (relationships with 0 training instance) and the few-shot setting (relationships with few training instances, \eg, $<10$), which reveals that by distilling linguistic knowledge into a deep model, we can dramatically improve the generalization of our data-driven model, which is hard to achieve by only training it on limited labeled images.



% By properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
% By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (\eg \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.











==> 906 2/intro.tex <==
\section{Introduction}
Detecting visual relationships from images is a central problem in image understanding.
% and a variety of high level computer vision applications, such as text-based image retrieval \cite{Johnson_2015_CVPR,li2016_3dscenefromtext}, visual question answering \cite{Sadeghi_2015_CVPR} and referring expression understanding \cite{varun}. 
Relationships are commonly defined as tuples consisting of a subject (\textit{subj}), predicate (\textit{pred}) and object (\textit{obj}) \cite{nlp1,nlp2,nlp3}. \textit{Visual} relationships represent the visually observable interactions between subject and object \twotup{subj}{obj} pairs, such as \threetup{person}{ride}{horse} \cite{VRD}. 

\begin{figure}[!t]
\centering
  \includegraphics[width=\linewidth]{images/system.pdf}
  \caption{Linguistic Knowledge Distillation Framework. We extract linguistic knowledge from training annotations and a public text corpus (green box), then construct a teacher network to distill the knowledge into an end-to-end deep neural network (student) that predicts visual relationships from visual and semantic representations (red box). GT is the ground truth label and ``+" is the concatenation operator.}
\label{fig:system}
\end{figure}

Recently, Lu \etal \cite{VRD} introduce the visual relationship dataset (VRD) to study learning of a large number of visual relationships from images. 
% Since it is difficult to collect a sufficiently large number of training images for all possible \threetup{subj}{pred}{obj} combinations, 
Lu \etal predict the predicates independently from the subjects and objects, and use the product of their scores to predict relationships present in a given image using a linear model.
% \begin{equation}
% \label{VRD_decompose}
% V(R|I)=P(subj)(\mathbf{w}^\intercal\textit{CNN}(I_{\text{union}})+b)P(obj)
% \end{equation}
% where $\textit{CNN}(I_{\text{union}})$ are the CNN features of a cropped image that contains the union of the two object bounding boxes. 
The results in \cite{VRD} suggest that predicates cannot be predicted reliably with a linear model that uses only visual cues, even when the ground truth categories and bounding boxes of the subject and object are given (\cite{VRD} reports Recall@100 of only 7.11\% for their visual prediction). Although the visual input analyzed by the CNN in \cite{VRD} includes the subject and object, predicates are predicted without any knowledge about the object categories present in the image or their relative locations. 
In contrast, we propose a probabilistic model to predict the predicate name jointly with the subject and object names and their relative spatial arrangement:
\begin{align}
\label{decompose}
P(R|I) =P(pred|I_{\text{union}},subj,obj)P(subj)P(obj).
\end{align}

While our method models visual relationships more accurately than \cite{VRD}, our model's parameter space is also enlarged because of the large variety of relationship tuples. This leads to the challenge of insufficient labeled image data. The straightforward---but very costly---solution is to collect and annotate a larger image dataset that can be used to train this model. Due to the long tail distribution of relationships, it is hard to collect enough training images for all relationships. To make the best use of available training images, we leverage linguistic knowledge (LK) to regularize the deep neural network. One way to obtain linguistic knowledge is to compute the conditional probabilities $P(pred|subj,obj)$ from the training annotations.
% which effectively model the strong correlation between \twotup{subj}{obj} pairs and predicates (\eg, if the subject and object were ``cup" and ``table", the predicate would be very likely be ``on"). We refer to the linguistic knowledge obtained from training annotations as ``internal knowledge".
% in the training set to regularize the deep neural network. 

% Another challenge is the linguistic data challenging. 
However, the number of \threetup{subj}{pred}{obj} combinations is too large for each triplet to be observed in a dataset of annotated images, so the internal statistics (\eg, statistics of the VRD dataset) only capture a small portion of the knowledge needed.
% potentially available.
To address this long tail problem, we collect external linguistic knowledge ($P(pred|subj,obj)$) from public text on the Internet (Wikipedia).
This external knowledge consists of statistics about the words that humans commonly use to describe the relationship between subject and object pairs,  and importantly, it includes 
% \twotup{subj}{obj} 
pairs unseen in our training data. Although the external knowledge is more general, it can be very noisy (\eg, due to errors in linguistic parsing). 

We make use of the internal and external knowledge in a teacher-student knowledge distillation framework \cite{eric1,eric2}, shown in Figure 1, where the output of the standard vision pipeline, called the \textit{student} network, is augmented with the output of a model that uses the linguistic knowledge to score solutions; their combination is called the \textit{teacher} network. 
% An additional term is then added to the standard loss function that penalizes divergence between student and teacher outputs. 
The objective is formulated so that the student not only learns to predict the correct one-hot ground truth labels but also to mimic the teacher's soft belief between predicates.

Our main contribution is that we exploit the role of both visual and linguistic representations in visual relationship detection and use internal and external linguistic knowledge to regularize the learning process of an end-to-end deep neural network to significantly enhance its predictive power and generalization. We evaluate our method on the VRD \cite{VRD} and Visual Genome (VG) \cite{VG} datasets. 
% Our method, utilizing only internal linguistic knowledge, significantly outperforms the state-of-the-art methods \cite{VRD,UIUC} (\eg, we achieve a Recall@100 of 29.89\% vs. 18.37\% in \cite{UIUC} on the VRD dataset for relationship detection).
% % With linguistic knowledge distillation, our method outperforms the purely data-driven baseline significantly (by 20.34\% Recall@100 for predicate detection). 
% Our student network obtains better generalization ability, especially in the zero-shot setting with unseen relationships (we improve predicate detection (Recall@100) from 8.45\% \cite{VRD} to 16.98\%). 
% Our evaluation of the combination of the internal and external linguistic knowledge suggests that we can train a student network that benefits from internal linguistic statistics for common visual relationships and from external statistics for long-tail relationships.
Our experiments using Visual Genome show that while the improvements due to training set size are minimal, improvements due to the use of LK are large, implying that with current dataset sizes, it is more fruitful to incorporate other types knowledge (\eg, LK) than to increase the  visual dataset size---this is particularly promising because visual data is expensive to annotate and there exist many readily available large scale sources of knowledge that have not yet been fully leveraged for visual tasks.





==> 906 2/intro_backup.tex <==
\section{Introduction}
Detecting visual relationships from images is a central problem in image understanding and a variety of high level computer vision applications, such as text-based image retrieval \cite{Johnson_2015_CVPR,li2016_3dscenefromtext}, visual question answering \cite{Sadeghi_2015_CVPR} and referring expression understanding \cite{varun}. Relationships are commonly defined as tuples of subject (\textit{subj}), predicate (\textit{pred}) and object (\textit{obj}) in natural language processing \cite{nlp1,nlp2,nlp3}. Similarly, visual relationships represent the visually observable interactions between subject and object \twotup{subj}{obj} pairs, such as \threetup{person}{ride}{horse} \cite{VRD}. 

\begin{figure}[!t]
\centering
  \includegraphics[width=\linewidth]{images/system.pdf}
  \caption{Linguistic Knowledge Distillation Framework. We extract linguistic knowledge from training annotations and other public text corpus (green box), then construct a teacher network to distill the knowledge into an end-to-end deep neural network (student) that predicts visual relationships from visual and semantic representations (red box). GT is the ground truth label. ``+" is the concatenation operator.}
\label{fig:system}
\end{figure}

Recently, Lu \etal \cite{VRD} introduced the visual relationship dataset (VRD) to study learning of a large number of visual relationships from images. 
% Since it is difficult to collect a sufficiently large number of training images for all possible \threetup{subj}{pred}{obj} combinations, 
Lu \etal predict the predicates independent from the subjects and objects, and use the product of their scores to predict relationships present in a given image using a linear model:
\begin{equation}
\label{VRD_decompose}
V(R|I)=P(subj)(\mathbf{w}^\text{T}CNN(I_{\text{union}})+b)P(obj)
\end{equation}
where $CNN(I_{\text{union}})$ are the CNN features of a cropped image that contains the union of the two object bounding boxes. 
The results in \cite{VRD} suggest that predicates cannot be predicted reliably with only visual module, even when the ground truth categories and bounding boxes of the subject and object are given (\cite{VRD} reports Recall@100 of only 7.11\% for their visual module). In \cite{VRD}, although the cropped image includes the subject and object, predicates are predicted without any knowledge about the object categories or relative locations. 
Thus, we propose a standard probabilistic model to predict the predicate name jointly with the subject and object names and their relative spatial arrangement:
\begin{align}
\label{decompose}
P(R|I) =P(pred|I_{\text{union}},subj,obj)P(subj)P(obj).
\end{align}

While the proposed method models visual relationships more accurately, the model's parameter space is also enlarged because of the large variety of relationship tuples. This leads to the visual data challenge of insufficient image data. The straightforward---but very costly---solution is to collect and annotate a larger image dataset that can be used to train this model. Due to the long tail distribution of relationships, it is hard to collect enough training images for all relationships. To make the most of available training images, we leverage linguistic knowledge (LK) to regularize the deep neural network. One way to obtain linguistic knowledge is to compute conditional probability of $P(pred|subj,obj)$ in the training annotations, which effectively models the strong correlation between \twotup{subj}{obj} pairs and predicates (e.g., if the subject and object were ``cup" and ``table", the predicate would be very likely to be ``on"). We denote the linguistic knowledge obtained from training annotations ``internal knowledge".
% in the training set to regularize the deep neural network. 

% Another challenge is the linguistic data challenging. 
Since the number of \threetup{subj}{pred}{obj} combinations is too large to be covered in a dataset of annotated images, the internal statistics (e.g., statistics of the VRD dataset) only capture a small portion of the knowledge in nature.
To address that problem, we collect external linguistic knowledge ($P(pred|subj,obj)$) from public texts on the Internet (Wikipedia) and distill it into the data-driven model. 
This external knowledge is extracted from a much larger and unconstrained domain and consists of statistics about which word humans commonly use to describe the relationship between a given subject and object pair, which hopefully includes unseen \twotup{subj}{obj} pairs in our training data. Although the external knowledge is more general, it can be very noisy (e.g., due to errors in linguistic parsing). Thus we combine the internal and external knowledge in a (multi-) teacher-student knowledge distillation framework shown in Figure \ref{fig:system}. 

We adopt a teacher-student framework \cite{eric1,eric2}, where the output of the standard deep vision pipeline, called the \textit{student} network, is augmented with the output of a model that uses the linguistic knowledge to score solutions, and their combination is called the \textit{teacher} network. 
An additional term is then added to the standard loss function that penalizes divergence between student and teacher outputs. 
The objective is formulated so that the student not only learns to predict the correct one-hot ground truth labels but also to mimic the teacher's soft belief between predicates.

Our main contribution is that we exploit the role of different visual and linguistic representations in visual relationship detection and use internal and external linguistic knowledge to regularize the learning process of an end-to-end deep neural network to significantly enhance its predictive power and generalization. We evaluate our contributions on the VRD \cite{VRD} and Visual Genome (VG) \cite{VG} datasets. For fair comparison, our method that utilizes only internal linguistic knowledge significantly outperforms the state-of-the-art methods \cite{VRD,UIUC} (e.g. we achieve a Recall@100 of 29.56\% vs. 18.37\% in \cite{UIUC} on VRD dataset for relationship detection).
With linguistic knowledge distillation, our method outperforms the pure data-driven baseline significantly (by 22.23\% Recall@100 for predicate detection). Our student network obtains better generalization ability, especially in the zero-shot setting with unseen relationships (we improve predicate detection (Recall@100) from 8.45\% \cite{VRD} to 15.53\%). Our experiments on the Visual Genome dataset shows that the while the improvements due to training set size are minimal, improvements due to the use of LK remain is large, implying that with current dataset sizes, it is more fruitful to incorporate additional knowledge (e.g., LK) than to increase the dataset size.
Our evaluation of the combination of the internal and external linguistic knowledge suggests that we can train a student network that benefits from internal linguistic statistics for common visual relationships and from external statistics for long-tail relationships.




==> 906 2/relatedWork.tex <==
\section{Related Work}
\textbf{Knowledge Distillation in Deep Neural Networks:} Recent work has exploited the use of additional information (or ``knowledge") to help train deep neural networks (DNN) \cite{k1,k2,k3,hinton}. Hinton \etal \cite{hinton} proposed a framework to distill knowledge, in this case the predicted distribution, from a large network into a smaller network. Recently, Hu \etal proposed a teacher-student framework to distill massive knowledge  sources, including logic rules, into DNNs \cite{eric1,eric2}.
% . Hu's framework constructs the teacher from the student to improve the of teacher during the learning process.

\textbf{Visual Relationship Detection:} Visual relationships represent the interactions between object pairs in images. Lu \etal \cite{VRD} formalized visual relationship prediction as a task and provided a dataset with a moderate number of relationships. Before \cite{VRD}, a large corpus of work had leveraged the interactions between objects (\eg object co-occurrence, spatial relationships) to improve visual tasks \cite{rich,o1,o2,o3,o4,o5,Ang}. 
% Visual phrases prediction \cite{VisualPhrase,vp} is similar to the VRD task, but the formulation of visual phrases limits the scale of relationships it can detect due to the large amount of labeled data for all possible combinations of predicates and objects.
To enable visual relationship detection on a large scale, Lu \emph{et al.} \cite{VRD} decomposed the prediction of a relationship into two individual parts: detecting objects and predicting predicates. Lu \emph{et al.} used the sub-image containing the union of two bounding boxes of object pairs as visual input to predict the predicates and utilized language priors, such as the similarity between relationships and the likelihood of a relationship in the training data, to augment the visual module. 

Plummer \emph{et al.} \cite{UIUC} grounded phrases in images by fusing  several visual features like appearance, size, bounding boxes, and linguistic cues (like adjectives that describe attribute information). Despite focusing on phrase localization rather than visual phrase detection, when evaluated on the VRD dataset,  \cite{UIUC} achieved comparable results with \cite{VRD}. Recently, there are several new attempts for visual relationship detection task:  Liang \etal \cite{RL} proposed to detect relationships and attributes within a reinforcement learning framework; Li \etal \cite{VIPCNN} trained an end-to-end system boost relationship detection through better object detection; Bo \etal \cite{Bo} detected relationships via a relational modeling framework.
% A more recent and larger dataset, Visual Genome [14] contains over 35K unique predicates and 2M relationship instances
% Aimed at detecting object part states, 
% Lu \emph{et al.} \cite{cewu} defined a pixel-wise annotation problem to infer rich semantic descriptions of objects at part level and tested their algorithm on a small set (6,429 out of 37,993 relationship instances, 31 out of 70 predicates) of the VRD dataset.
% Lu \emph{et al.} extracted the part state binary vectors (\eg ``hand holds something" is one part state) of two objects, and concatenated them as features of a SVM model, then averaged the SVM scores with the ones that calculated based on the method in \cite{VRD} as their final results. 
% One limitation of their method is that it requires a lot of human efforts on defining part states (856 part states of 15 object categories in \cite{cewu}) and a large number of training data when facing with relationship detection tasks with more objects.
% Our proposed method exploits the strong linguistic correlation between the predicate and \twotup{subj}{obj} pairs and the spatial relationship between the two bounding boxes. 
% While Lu \etal \cite{VRD} utilized similarity between relationships and the likelihood of \threetup{subj}{pred}{obj} combinations to train a linear language model, they resorted to a simple product of two linear model (visual and language) as their final prediction results. In contrast, we 
% combine rich visual and linguistic representations in an end-to-end deep neural network that absorbs external linguistic knowledge using the teacher-student framework during training process to enhance prediction and generalization ability. Unlike \cite{hinton,eric1,eric2}, which used either the teacher or the student as their final output, we combine both teacher and student networks, as they each have their own advantages: the teacher outperforms in cases with sufficient training data, while the student generalizes to cases with few or no training examples (the zero-shot case).

% Different from the existing methods, 
We combine rich visual and linguistic representations in an end-to-end deep neural network that absorbs external linguistic knowledge using the teacher-student framework during the training process to enhance prediction and generalization.  Unlike \cite{VRD}, which detected objects independently from relationship prediction, we model objects and relationships jointly. Unlike \cite{VIPCNN,RL,Bo}, which do not use linguistic knowledge explicitly, we focus on predicting predicates using the linguistic knowledge that models correlations between predicates and \twotup{subj}{obj} pairs, especially for the long-tail relationships. Unlike \cite{hinton,eric1,eric2}, which used either the teacher or the student as their final output, we combine both teacher and student networks, as they each have their own advantages: the teacher outperforms in cases with sufficient training data, while the student generalizes to cases with few or no training examples (the zero-shot case).

==> Sup.tex <==

\section{Semantic and Spatial Representations}

Spatial features have been demonstrated to be helpful in visual tasks such as object detection, image retrieval and semantic segmentation \cite{rich,o1,o2,o3,o4,o5,Ang}. For visual relationship detection task,
spatial features such as the relative location and size of two objects are informative for predicate prediction. For example, relative location is a discriminative feature for predicates ``under" and ``above" of the VRD training set shown in Figure \ref{fig:under} and \ref{fig:above}. To explicitly model the spatial location and size of an object,  we use the features from \cite{varun}:
\begin{equation}
\label{Spatial_Feature}
\left[\frac{x_{min}}{W},\frac{y_{min}}{H},\frac{x_{max}}{W},\frac{y_{max}}{H},\frac{A}{A_{img}}\right]
\end{equation}
where $W$ and $H$ are the width and height of the image, $A$ and $A_{img}$ are the areas of the object and the image, respectively. We concatenate the above features of two objects as the spatial feature (SF) for a \twotup{subj}{obj} pair. 


% \begin{figure}
% \centering     
% \subfigure[Number of \twotup{subj}{obj} Pairs vs. Number of Possible Predicates]{\label{fig:NI_Entropy}\includegraphics[width=40mm]{images/Pair.pdf}}
% \subfigure[Example to illustrate LK Distillation.]{\label{fig:example}\includegraphics[width=40mm]{images/cropped_sample}}
% \caption{(a). Most of the \twotup{subj}{obj} pairs has very a limited number of predicates that are used to describe their relationship. (b). The top-right distribution is the output of the student network; the bottom-right one is the teacher's output after penalizing the unlikely predicates given the \twotup{subj}{obj} pair.}
% \end{figure}

\begin{figure}[b]
\centering
  \includegraphics[width=70mm]{images/Pair.pdf}
  \caption{Number of \twotup{subj}{obj} Pairs vs. Number of Possible Predicates}
\label{fig:NI_Entropy}
\end{figure}

\begin{figure}[t]
\centering     
\subfigure[under]{\label{fig:under}\includegraphics[width=20mm]{images/under.eps}}
\subfigure[above]{\label{fig:above}\includegraphics[width=20mm]{images/above.eps}}
\subfigure[on]{\label{fig:on}\includegraphics[width=20mm]{images/on.eps}}
\subfigure[in]{\label{fig:in}\includegraphics[width=20mm]{images/in.eps}}
\caption{Relative location of subjects and objects for different predicates. Red box (coordinates normalized as $[0,0,1,1]$ for $[x_1,y_1,x_2,y_2]$) is the subject, blue boxes are the objects. Predicates like ``under" and ``above" are discriminative based on relative location. However, ``on" and ``in" are different to distinguish.}
\end{figure}

Given a fixed \twotup{subj}{obj} pair, only a few predicates are relevant, something which emerges by a simple analysis of linguistic descriptions of objects and their relationships. Considering that most of the \twotup{subj}{obj} pairs of the VRD training dataset have a limited number of relevant predicates.
% which indicates that given \twotup{subj}{obj} pairs, the number of plausible predicates is very limited. 
The strong correlation between a predicate and the \twotup{subj}{obj} pairs indicates that the semantic object representation  (a description of its type or class) should be informative for relationship detection, especially when the spatial features are ambiguous for different predicates. For instance, the relative bounding box locations of the subject and object \wrt predicate ``on" and ``in" as shown in \ref{fig:on} and \ref{fig:in} are similar, but given a subject of type "plate" and an object of type ``table", common sense predicts ``on" as the predicate. 
% Unlike \cite{VRD} which utilized the likelihood of \threetup{subj}{pred}{obj} combinations in their language module, our semantic representation that considers only the objects is more general.


% We predict the predicate conditioned on the semantic and spatial representations of the subject and object:
% \begin{align}
% \label{decompose}
% P(R|I) =&P(pred|subj,obj,B_s,B_o,I)\nonumber \\
% &~~\cdot P(subj,obj,B_s,B_o|I)
% \end{align}
% where $subj$ and $obj$ are represented using the semantic object representation (word2vec \cite{word2vec} is used and confidence score distribution is obtained from object detection), $B_s,B_o$ are the spatial features and $I$ is the image region of the union of the two bounding boxes.



\subsection{Evaluation of Semantic and Spatial Representations}
We evaluate the use of semantic object representations and the spatial features without LK distillation. We compare our method with three methods in \cite{VRD} and \cite{VisualPhrase}: ``Visual Phrases" denotes the method that trains deformable parts models for each relationships; ``Joint CNN" denotes the method trains a 270-way CNN model to predict the subject, object and predicate together. ``VRD - V only" denotes the method proposed in \cite{VRD} that uses VGG-net to extract features for the BB-Union of two bounding boxes and then feeds the features into a learned linear model to predict the predicate. Besides the existing methods, we also compare our method with a baseline that uses the same VGG-net as \cite{VRD} and BB-Union of boxes but with end-to-end training  (denoted as ``Baseline: U"). To test the use of our semantic and spatial features, we test different combinations, shown in Table \ref{P:visual} and Table \ref{P:visualZero}. 

\begin{table}[t]
\centering
\caption{Predicate Detection: Different Visual Features. ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``one-hot" and ``word2vec" are two semantic representations.}
\label{P:visual}\vskip 3pt
% \resizebox{\textwidth}{!}
% \footnotesize
\scriptsize
%\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
                    & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.},                                & R@100,                 & R@50,                                  \\
& k=1                                       & k=70                   & k=70                   \\\midrule
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -          \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -          \\
VRD - V only  \cite{VRD}        & 7.11             & 37.20           & 28.36          \\
% Linguistic Cues       & -          & -         & -           & -          \\
\midrule
Baseline: U                 & 34.82          & 83.15       & 70.02      \\
U + one-hot        & 36.42           & 84.66       & 71.07      \\
U + word2vec      & 37.15          & 83.78       & 70.75      \\
U + SF            & 36.33           & 83.68       & 69.87           \\
U + one-hot + SF   & 38.87           & 84.34       &71.79      \\
U + word2vec + SF & \textbf{41.33}          & \textbf{84.89}       &  \textbf{72.29}      \\ \bottomrule
\end{tabular}
\end{table}

Table \ref{P:visual} reveals that end-to-end training (our ``Baseline: U ") with soft-max prediction outperforms the feature+linear model method (``VRD - V only"), highlighting the importance of fine-tuning. In addition, adding semantic or spatial features individually improves the predictive power of the data-driven model. The combination of BB-Union, semantic and spatial features yields the best performance. 

We report the performance of different methods on zero-shot predicate prediction task in Table \ref{P:visualZero}. Our end-to-end CNN model using BB-Union, semantic and spatial features outperforms \cite{VRD} by a large margin in the zero-shot setting. Among the three sets of features, the spatial feature generalizes best, the one-hot feature the worst, the word2vec feature in between. We believe that this is because some \twotup{subj}{obj} pairs in the zero-shot setting never occur in the training set, and the one-hot feature is too specific to generalize from the seen pairs to the unseen pairs. 
The word2vec features generalize better because the formulation of the vector space already takes the semantic similarity of different objects into consideration. 
% Since the zero-shot setting is only on semantic level, 
Spatial features that capture low level information of bounding boxes generalize the best.

\begin{table}[]
\centering
\caption{Predicate Detection: Different Visual Features - Zero Shot. We use the same notations as in Table \ref{P:visual}.}\vskip 3pt
\label{P:visualZero}
% \footnotesize
\scriptsize
%\setlength\tabcolsep{2.5pt}
\begin{tabular}{@{}lccc@{}}
\toprule
                      & R@100/50,                                 & R@100,                 & R@50,                                  \\
& k=1                                     & k=70                   & k=70                   \\\midrule
VRD - V only \cite{VRD}               & 3.52      & 32.34           & 23.95          \\ 
% Linguistic Cues       & -          & -         & -           & -          \\
\midrule
Baseline: U                     & 12.75     & 69.42       & 47.84      \\
U + one-hot            & 11.86     & 69.46       & 47.22      \\
U + word2vec           & 13.44     & \textbf{69.77}       & \textbf{49.01}      \\
U + SF                & \textbf{14.33}     & 69.01       & 48.32      \\
U + one-hot + SF        & 12.98     & 69.35       & 48.79      \\
U + word2vec + SF       & 14.13     & 69.41       & 48.13      \\ \bottomrule
\end{tabular}
\end{table}

\subsection{When do Spatial Features Help?}
To show the role of spatial features in visual relationship detection task, We observe from Figure \ref{fig:NI_Entropy} that most of the \twotup{subj}{obj} pairs have low entropy in their predicate distribution, which implies a strong correlation between a predicate and \twotup{subj}{obj} pairs. It is interesting to understand why adding the spatial features outperforms a model that already knows which objects it is analyzing. We choose the method ``U + word2vec + SF" and ``U + word2vec" to evaluate when spatial features help. Our hypothesise is that SF helps when \twotup{subj}{obj} is not very deterministic. 
% One measurement to model the uncertainty of the predicate given \twotup{subj}{obj} is the entropy of predicate distribution. 
We plot the ``R@100/50, k=1" improvement of ``U + word2vec + SF" over ``U + word2vec" vs. the entropy of $P(pred|subj,obj)$ in Figure \ref{fig:Entropy}.

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\linewidth]{images/Entropy.eps}
%   \caption{R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$}
% \label{fig:Entropy}
% \end{figure}

% \begin{figure}
% \centering     
% \subfigure[ ]{\label{fig:Entropy}\includegraphics[width=40mm]{images/Entropy.eps}}
% \subfigure[ ]{\label{fig:im}\includegraphics[width=40mm]{images/Improve_number_histo.pdf}}
% \caption{(a). R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$ (b). Recall@100 Improvement with LK-distillation vs. the number of training \twotup{subj}{obj} pairs.}
% \end{figure}

\begin{figure}[t]
\centering
  \includegraphics[width=70mm]{images/Entropy.eps}
  \caption{R@100, k=1 improvement vs. Entropy of $P(pred|subj,obj)$}
\label{fig:Entropy}
\end{figure}

% \begin{figure}[t]
% \centering
%   \includegraphics[width=\linewidth]{images/Improve_number_histo.pdf}
%   \caption{Recall@100 Improvement with LK-distillation vs. the number of training \twotup{subj}{obj} pairs.}
% \label{fig:im}
% \end{figure}



We notice that when the entropy is small (\twotup{subj}{obj} is deterministic), most of the relationships with those \twotup{subj}{obj} pairs do not benefit from adding spatial features. However, when the entropy is large (1-1.5), adding spatial features improves predictive power for those relationships. 



% \subsubsection{Knowledge Transfer with Linguistic Knowledge Distillation}

% One application of our LK distillation framework is that if we can obtain reasonable good linguistic knowledge, we can use very limited training data to obtain 

% \begin{table}[]
% \centering
% \caption{Knowledge Transfer: Train on VRD dataset with the linguistic knowledge from VG; test on VG dataset. We use the same notations as in Table \ref{VG}.}
% \label{transfer}\vskip 3pt
% % \footnotesize
% \scriptsize
% \setlength\tabcolsep{5pt}
% \begin{tabular}{@{}lccc@{}}
% \toprule
%                                  & R@100/50,                               & R@100,                 & R@50,                                  \\
% & k=1                                 & k=70                   & k=70                   \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Train and test on VG}} \\
% U+W+SF               & 40.62    & 86.65    & 83.91       \\
% U+W+SF+L: S         & 49.88    & 91.25    & 88.14      \\
% U+W+SF+L: T         & 55.02    & 94.92    & 91.47       \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 2: Train on VRD with LK from VG; test on VG}} \\
% U+W+SF               & 32.08    & 78.43    & 72.46       \\
% U+W+SF+L: S         & 45.89    & 91.32    & 82.73      \\
% U+W+SF+L: T         & 52.26    & 94.06    & 90.53       \\\midrule

% \end{tabular}
% \end{table}

\section{Linguistic Knowledge Distillation with More Training Images} 
Another interesting finding is that LK-distillation offers higher performance improvement for the relationships that  have few training instances, which is also reported in \cite{eric2} (details can be found in the supplementary materials). This observation supports our motivation that knowledge helps the long-tail relationships most.

A natural question is: can we just collect more data and obtain significant improvement in predictive power and generalization? To answer this question, we utilize the recently proposed Visual Genome dataset \cite{VG} to augment the training data of VRD. By selecting the relationship instances and have predicates and objects in the categories of VRD dataset from images that are not in VRD set from Visual Genome set, we obtain around 130K more training instances, enlarging the original VRD training set by 5$\times$. To make the zero-shot testing set of VRD remain unseen, we ensure that the relationships in the zero-shot set are excluded from the augmented training data. We conduct similar experiments with the augmented dataset and distill the same linguistic knowledge extracted from VRD dataset. The results are shown in the Part 2 of 
Table 1, 2 and 3 in the main paper. 
We observe that training with more data leads to only marginal performance improvement of almost all baselines and proposed methods. However, for all experimental settings, with more data, our LK distillation framework still brings significant improvements, and the combination of the teacher and student networks still yields the best performance. The experiments imply that simply adding more training images does not help much. One reason we observe is that the distribution of relationships in the newly added images are still long-tail (although the Visual Genome dataset is much larger than VRD), the data-driven model still does not get enough training data. Another reason is that since we still use the linguistic knowledge extracted from VRD set, the strong linguistic prior dominates the predictions so that we observe the performance of teacher networks are very similar with/without the newly added images from Visual Genome dataset. Both reasons imply that we may need to extract the linguistic knowledge from a larger domain that contains more unseen relationships.

% \begin{table}[]
% \centering
% \scriptsize
% \setlength{\tabcolsep}{3.5pt} 
% \caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them. \textbf{Part 1} uses the training images in VRD dataset and \textbf{Part 2} uses the training images in VRD \cite{VRD} and all images of Visual Genome (VG) \cite{VG} dataset.}
% \label{P_VRD_1}
% \begin{tabular}{@{}lccc|ccc@{}}
% \toprule
% \multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
% \multicolumn{1}{@{}l}{ } & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
% \multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}} &&&& \\
% Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
% Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

% VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
% VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

% Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
% Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
% U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
% U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
% U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
% U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
% U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
% U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
% U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
% U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
% U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
% U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\\midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
% \bottomrule
% \end{tabular}
% \end{table}




% \begin{table*}[t]
% \centering
% \caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD_1}.}\vskip 3pt
% \label{Detection_1}
% % \footnotesize
% \scriptsize
% \setlength\tabcolsep{3.5pt}
% \begin{tabular}{@{}lcccccc|cccccc@{}}
% \toprule
% & \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% % \textbf{Part 1: VRD only} 
% & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
% & k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}}&&&&&&&&&&\\
% VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
% Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
% U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
% U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
% U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\

% \end{tabular}
% \end{table*}



% \begin{table*}[t]
% \centering
% % \footnotesize
% \scriptsize
% \caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD_1}.}\vskip 3pt
% \setlength\tabcolsep{3.8pt}
% \label{Detection_Zero_1}
% \begin{tabular}{@{}lcccccc|cccccc@{}}
% \toprule
%                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
%                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
%                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{\textbf{Part 1: Training images VRD only}}&&&&&&&&&&\\

% VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
% Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
% U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
% U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\


% \end{tabular}
% \end{table*}



==> exp_back.tex <==
\section{Experiments}\label{exp}
\subsection{Dataset}
We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
%   \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
%   \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
% \end{itemize}


\subsection{Implementation Details}
We use VGG-net \cite{VGG} to learn the visual representations of the BB-Union of two objects. For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, we use a pre-trained word2vec model to project the subjects and objects into vector space, and the final representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\subsection{Evaluation Metric}
We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in VRD is not exhaustive \cite{VRD}).
The standard Recall@n metric ranks all predictions for an image and choose the top n predictions. However, \cite{VRD} evaluated only the top prediction for each pair, and rank the predictions for all pairs in a image, then ranked these select the top n to report the Recall@n. By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
Considering multiple predicates can correctly describe the same object pair, (e.g. when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
we believe that a good predicted probability distribution of a predicate that captures the semantic similarity between plausible predicates should has large probability of plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalizes correct predictions because of the annotator's preference or random choice from several plausible predicates. 
% Since there are multiple pairs of objects in an image, and each pair has 70 predictions with different confidence scores, 

We treat the number of chosen predictions per pair (k) as a hyper-parameter, and report R@n for two different $k$'s: 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}



\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our proposed method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate our method given ground truth object detection results, which is the predicate prediction tasks in \cite{VRD}. Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. Since \cite{UIUC} does not report the results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}.

Table \ref{P_VRD} show the evaluation of linguistic knowledge distillation with different set of features in our deep neural networks. In addition to the data-driven baseline, we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". ``Visual Phrases" denotes the method that trains deformable parts models for each relationships \cite{VisualPhrase}; ``Joint CNN" denotes the method trains a 270-way CNN model to predict the subject, object and predicate together. The visual model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". In both tables, S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline that uses the same visual representation (BB-Union) as \cite{VRD} and the ``VRD-V only" model, the huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 31.62\% (ours)) reveals that the end-to-end training with soft-max prediction outperforms the extracting feature from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding semantic representation and spatial features improves the predictive power and generalization of the data-driven model. More analysis on using different combination of features can be found in the supplementary materials.



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{} &&&& \\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\
% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships in training data]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Unseen relationships in training data]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of Predicate Detection: Different Methods. ``Data-driven" denotes the Baseline: U; ``LK only" denotes the Baseline: L only; ``Full model student" denotes the U+W+SF+LK: S; ``Full model teacher" denotes the U+W+SF+LK: T.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\

VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\

\bottomrule


\end{tabular}
\end{table*}


To demonstrate the effectiveness of our LK-distillation framework, we compare the results of using different combinations of features with/without using LK-distillation. In Part 1 of table \ref{P_VRD}, for fair comparison with the existing methods, we train and test our model on VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the data-driven baseline all of the state-of-the-art methods (\cite{VisualPhrase}, \cite{Rcnn} and \cite{VRD}) by a large margin (e.g. 51.34\%  vs. 47.87\% \cite{VRD} for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without even looking at the images leads to very pool performance on the zero-shot set of VRD, which implies the poor generalization of ``Baseline: L only" method and addresses the need of combining both data-driven and knowledge-based method as the LK-distillation framework we propose.

To show the benefit of LK-distillation, we observe a consistent trend that for all feature settings, the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models by a large margin, (e.g. R@100/50, k=1 is improved from 33.48\% to 40.95\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in training data; the other is that although the linguistic priors are powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far away from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels be equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin (e.g. 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework have their own advantages. The best predictive power is achieved when we combine them together: we use teacher's network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. Setting ``U+W+SF+LK: T+S" achieves the best performance. One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. Visualizations of different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we follow \cite{VRD} to use a R-CNN based detector \cite{Rcnn} for object detection tasks. Given the confidence scores of each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution of each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with methods in \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report the recall. In addition, we report the standard recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Part 1 of Table \ref{Detection} and \ref{Detection_Zero}. 

We observe that our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} by a large margin on both entire testing set and the zero-shot setting. The observations about student and teacher networks are consistent with the ones in predicate prediction evaluation. On the other hand, when comparing the results of predicate and relationship prediction, the large performance margin (53.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental task such as object detection.

\subsection{Evaluation on Visual Genome Dataset}

To show our generic framework works on different data distribution, we evaluate our method on Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct similar evaluation on this much larger dataset (99,864 relationship instances for training and  19,754 for testing. In the testing set, 2,056 relationships instance are never seen in the training data.) using the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar results as our experiments on VRD dataset that the LK distillation method manages to regularize the learning process of the deep model and improve its predictive power and generalization. We also conduct another experiment that we use images in Visual Genome dataset to augment the training set of VRD and still test on VRD dataset. When the R@100/50 k=1 of pure data-driven model for predicate detection is improved from 31.62\% to 33.67\% due to a larger training set, our LK-distillation boosts the recall to 53.38\%, which reveals that incorporating additional knowledge brings more benefits than collecting more data. More details can be found in the supplementary materials. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset: We use the same notations as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 36.83    & 83.05    & 81.38    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.62    & 86.65    & 83.91    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits from extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
For those unseen long-tail relationships in VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results using our linguistic knowledge distillation framework, then testing on VRD dataset with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, an interesting finding is that, although the external knowledge can be very noisy (Wikipedia) or has a different distribution when compared with the VRD dataset (Visual Genome), the performance of teacher network using external knowledge is much better than the one restricted in the VRD training dataset (Part 1). 
That finding suggests that by properly distilling the external knowledge, our framework may manage to obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 

To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. \textbf{Part 1} uses the LK from VRD dataset; \textbf{Part 2} uses the LK from VG dataset; \textbf{Part 3} uses the LK from both VRD and VG dataset. \textbf{Part 4} uses the LK from parsing Wikipedia text; \textbf{Part 5} uses the LK from from both VRD dataset and Wikipedia. We use the same notations as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\textbf{Part 1 LK: VRD}  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S         & 45.50    & 85.67    & 74.98    & 15.53   & 71.15    & 52.21  \\
U+W+SF+L: T         & 53.03    & 88.43    & 81.78    & 8.30    & 40.03    & 31.31   \\\midrule
\textbf{Part 2 LK: VG} & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 15.31   & 69.29    & 48.59   \\
U+W+SF+L: T         & 51.00    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{\textbf{Part 3 LK: VRD+VG}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 16.88    & 74.09   & 54.29   \\
U+W+SF+L: T         & \textbf{53.67}    & \textbf{90.13}    & \textbf{83.63}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 4 LK: Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 5 LK: VRD+Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 47.64   & 88.21   & 77.79    & \textbf{18.17}    & \textbf{75.62}    & \textbf{56.45}   \\
U+W+SF+L: T         & 52.14    & 88.23   & 81.78    & 8.95     & 39.24   & 30.61  \\\bottomrule
\end{tabular}
\end{table}


We observe that by properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (e.g. \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.







==> exp_back_0309.tex <==
\section{Experiments}\label{exp}
% We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
We evaluate our LK-distillation method on the Visual Relationship Detection \cite{VRD} and Visual Genome \cite{VG} datasets. There are three evaluation tasks:
% 1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
% 2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
% 3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\begin{itemize}
\itemsep -1pt
  \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
  \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
  \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\end{itemize}

Both datasets have a zero-shot testing set that contains relationships that never occur in the training data. We also evaluate our approaches on the zero-shot sets to demonstrate the improvement on generalization by linguistic knowledge distillation.

\textbf{Implementation Details.} We use VGG-net \cite{VGG} to learn the visual representations of the BB-Union of two objects. For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. 
% For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, 
We use a pre-trained word2vec model to project the subjects and objects into vector space, and the final semantic representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\textbf{{Evaluation Metric.}} We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in the datasets are not exhaustive).
For two detected objects, there can be multiple predicate predictions with different confident scores. The standard Recall@n metric ranks all predictions for all detected object pairs in an image and chooses the top n predictions to compute the recall. However, in contrast of computing recall based on all predictions, \cite{VRD} evaluated only the prediction with highest confident score for each object pair. 
By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
However, considering the fact that multiple predicates can correctly describe the same object pair, (e.g., when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
we believe that a good predicted probability distribution of a predicate that captures the semantic similarity between plausible predicates should have large probability for plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalize correct predictions because of the annotator's preference or random choice amongst several plausible predicates. 
% Since there are multiple pairs of objects in an image, and each pair has 70 predictions with different confidence scores, 

We treat the number of chosen predictions per object pair (k) as a hyper-parameter, and report R@n for different $k$'s to compare with other state-of-the-art methods \cite{VRD,UIUC,VisualPhrase}. Since the number of predicates is 70, $k=70$ is equivalent to getting every predictions of two detected objects into evaluation. 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
% 1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
% 2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}

\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate it given ground truth object detection results, which is the predicate prediction task in \cite{VRD}. 
% Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. 
Since \cite{UIUC} does not report results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}.

Table \ref{P_VRD} shows the evaluation of linguistic knowledge distillation with different sets of features in our deep neural networks. In addition to the data-driven baseline ``Baseline: U only", we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". The "Visual Phrases" method \cite{VisualPhrase} trains deformable parts models for each relationships ; ``Joint CNN" \cite{Rcnn} trains a 270-way CNN model to predict the subject, object and predicate together. The visual model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline that uses the same visual representation (BB-Union) as \cite{VRD} and the ``VRD-V only" model, the huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 31.62\% (ours)) reveals that the end-to-end training with soft-max prediction outperforms extracting features from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding the semantic representation and the spatial features improves the predictive power and generalization of the data-driven model. \footnote{More analysis on using different combinations of features can be found in the supplementary materials.}



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
% \multicolumn{3}{@{} l}{} &&&& \\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20\tablefootnote{The results of Recall when k=70 are not reported in \cite{VRD}. To show the improvement of our method with different k's we calculate those recall values using their code. The same for Table \ref{Detection} and \ref{Detection_Zero}.}           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 31.62     & 82.35       & 68.12    & 11.72     & 68.12       & 46.54   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 33.48     & 84.28       & 69.35   & 12.64     & 70.37       & 49.37    \\
U+W+L:S               & 40.95     & 86.14       & 72.73  & 13.69       & 71.03       & 50.17     \\
U+W+L:T               & 52.65     & 88.08       & 82.16   & 6.84          & 39.69       & 31.22   \\\hdashline
U+SF                 &32.33           & 81.98       & 66.85  & 13.73     & 67.03       & 47.32    \\
U+SF+L:S                       & 36.06     & 83.83       & 69.26    & 14.24          & 69.72       & 49.62  \\
U+SF+L:T               & 50.37     & 87.01       & 80.24     & 7.01          & 39.61       & 29.77    \\ \hdashline
U+W+SF+L                    & 39.03     & 84.37       & 70.29  & 13.43         & 66.81       & 47.13    \\
U+W+SF+L: S            & 45.50      & 85.67       & 74.98  & \textbf{15.53}       & \textbf{71.15}       & \textbf{52.21}    \\
U+W+SF+L: T          & 53.03     & 88.43       & 81.78   & 8.30           & 40.03       & 31.31    \\
U+W+SF+L: T+S    & \textbf{53.85}     & \textbf{93.55}       & \textbf{84.34}    & -          & -       & -  \\
% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}
%                                               & & &  &                      \\
% Baseline: U                                           & 33.67     & 84.40  & 69.29   & 11.98     & 69.72  & 49.53     \\
% U+W+SF                     & 38.28     & 85.62       & 71.43   & 13.60          & 70.49       & 50.04     \\
% U+W+SF+L: S             & 48.00      & 86.45       & 74.90    & 15.83           & 71.26       & 52.90     \\
% U+W+SF+L: T             & 53.38     & 89.09       & 82.27       & 8.73          & 40.21       & 31.48   \\
% U+W+SF+L: T+S               & 54.02     &94.51      & 85.31    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships in training data]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Unseen relationships in training data]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of predicate detection results: ``Data-driven" denotes the baseline using BB-Union; ``LK only" denotes the baseline using only the linguistic knowledge without looking at the image; ``Full model student" denotes the student network with U+W+SF features; ``Full model teacher" denotes the teacher network with U+W+SF features.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \midrule%\hdashline
U+W+SF+L: S      & 18.68 & 17.27 & 22.76 & 19.83 & 22.64	& 19.67 & 16.50 & 15.17 & 27.53 & 17.68 &28.75	&16.51\\
U+W+SF+L: T      & 19.15 & 17.60 & 25.74 & 21.36 &25.56	&21.46 & 17.11 & 15.79 & 29.24 & 18.19 &31.47	&18.26\\
U+W+SF+L: T+S  & \textbf{19.48} & \textbf{18.11} & \textbf{26.04} & \textbf{21.87} &\bf25.91	&\bf21.67 & \textbf{17.30} & \textbf{15.91} & \textbf{29.56} & \textbf{18.55} &\bf 31.75	&\bf18.68\\

% \midrule

% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 18.92 & 17.56 & 23.19 & 20.04 & 23.27	& 19.93 & 16.71 & 15.43 & 28.31 & 17.82 &29.85	&16.88\\
% U+W+SF+L: T      & 19.38 & 18.29 & 25.83 & 21.70 &25.92	&21.65 & 17.19 & 16.21 & 29.46 & 18.79 &31.84	&18.64\\
% U+W+SF+L: T+S     & 19.76 & 18.51 & 26.13 & 21.93 &26.05	&21.98 & 17.35 & 16.67 & 29.95 & 19.14 &32.06	&18.98\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
% \multicolumn{3}{@{} l}{}&&&&&&&&&&\\

VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\midrule%\hdashline
U+W+SF+L: S   & \textbf{7.61} & \textbf{7.29} & \textbf{16.67} & \textbf{12.43} &\bf 16.34	&\bf 12.28 & \textbf{6.59} & \textbf{6.33} & \textbf{15.48} & \textbf{11.41} &\bf 14.71	&\bf 9.50\\ 	
U+W+SF+L: T  & 3.59 &3.51 & 10.61 & 8.21  & 9.58 &7.44 & 3.25 & 3.17 & 9.82  & 7.68 & 8.73	&6.84\\
% \midrule
   
% \multicolumn{3}{@{} l}{\textbf{Part 2: Training images VRD + VG}}&&&&&&&&&&\\
% U+W+SF+L: S      & 7.73 & 7.60 & 16.78 & 12.63 & 16.88	& 12.65 & 6.76 & 6.43 & 15.60 & 11.68 &15.37	&10.52\\
% U+W+SF+L: T      & 3.74 & 3.61 & 10.27 & 8.30 &9.84	&7.86 & 3.17 & 3.13 & 9.71 & 7.82 &9.07	&7.19\\

\bottomrule


\end{tabular}
\end{table*}

To demonstrate the effectiveness of our LK-distillation framework, we compare the results of using different combinations of features with/without using LK-distillation. In table \ref{P_VRD}, for fair comparison with existing methods, we train and test our model on the VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the state-of-the-art method \cite{VRD} by a large margin (e.g., 51.34\%  vs. 47.87\% for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without even looking at the images leads to very pool performance on the zero-shot set of VRD, which explains the poor generalization of ``Baseline: L only" method and addresses the need for combining both data-driven and knowledge-based methods as the LK-distillation framework we propose does.

To show the benefit of LK-distillation, we observe a consistent trend that for all feature settings, the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models significantly (e.g., R@100/50, k=1 is improved from 33.48\% to 40.95\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in the training data; the other is that although the linguistic prior is powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on the zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin (e.g., 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework have their own advantages. The best predictive power is achieved when we combine them together: we use the teacher network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. The setting ``U+W+SF+LK: T+S" achieves the best performance. 
% One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. 
Visualizations of the different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we follow \cite{VRD} to use an R-CNN based detector \cite{Rcnn} for object detection tasks. Given the confidence scores of each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution for each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report the recall. In addition, we report the standard recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Tables \ref{Detection} and \ref{Detection_Zero}. 

Our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} significantly on both entire testing set and zero-shot setting. The observation about student and teacher networks are consistent with predicate prediction evaluation. Additionally, when comparing the results of predicate and relationship prediction, the large performance gain (53.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental object detection task.

\subsection{Evaluation on Visual Genome Dataset}

We also evaluate our method on the Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations, on the predicate detection task. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct similar evaluation on the dataset (99,864 relationship instances in training and 19,754 in testing. In the testing set, 2,056 relationships instance are never seen in the training data). We use the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar behavior as our experiments on the VRD dataset--LK distillation manages to regularize the deep model and improve its generalization. We conduct another experiment in which images from Visual Genome dataset augment the training set of VRD and evaluate on the VRD test set\footnote{Details can be found in the supplementary materials.}. While the R@100/50 k=1 measure of the purely data-driven model for predicate detection improves from 31.62\% to 33.67\% due to the increased training size, our LK-distillation boosts recall to 53.38\%, which reveals that incorporating additional knowledge is more beneficial than collecting more data. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset. Notations are the same as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 36.83    & 83.05    & 81.38    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.62    & 86.65    & 83.91    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits of extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
% However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
However, training annotations only represent a small portion of all possible relationships and do not necessarily represent the real world distribution, which is essentially long tail.
For those unseen long-tail relationships in the VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results on the VRD test set using our linguistic knowledge distillation framework with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, interestingly, although the external knowledge can be very noisy (Wikipedia) or have a different distribution when compared with the VRD dataset (Visual Genome), the performance of the teacher network using such external knowledge is much better than that restricted to the VRD training dataset (Part 1). 
This finding suggests that by properly distilling the external knowledge, our framework can obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 
% To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
% After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
% The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
% We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. We observe that by distilling external knowledge with the internal one, we improve the generalization significantly (e.g., LK from Wikipedia boosts the recall to 18.17\% on the zero-shot set) while maintaining good predictive power on the entire test set.

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. \textbf{Part 1} uses the LK from VRD dataset; \textbf{Part 2} uses the LK from VG dataset; \textbf{Part 3} uses the LK from both VRD and VG dataset. \textbf{Part 4} uses the LK from parsing Wikipedia text; \textbf{Part 5} uses the LK from from both VRD dataset and Wikipedia. Notations are the same as as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\textbf{Part 1 LK: VRD}  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S         & 45.50    & 85.67    & 74.98    & 15.53   & 71.15    & 52.21  \\
U+W+SF+L: T         & 53.03    & 88.43    & 81.78    & 8.30    & 40.03    & 31.31   \\\midrule
\textbf{Part 2 LK: VG} & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 15.31   & 69.29    & 48.59   \\
U+W+SF+L: T         & 51.00    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{\textbf{Part 3 LK: VRD+VG}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 16.88    & 74.09   & 54.29   \\
U+W+SF+L: T         & \textbf{53.67}    & \textbf{90.13}    & \textbf{83.63}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 4 LK: Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{\textbf{Part 5 LK: VRD+Wiki}} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 47.64   & 88.21   & 77.79    & \textbf{18.17}    & \textbf{75.62}    & \textbf{56.45}   \\
U+W+SF+L: T         & 52.14    & 88.23   & 81.78    & 8.95     & 39.24   & 30.61  \\\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
  \includegraphics[width=60mm]{images/I_N}
  \caption{Performance with varying sizes of training examples. ``Our Method" denotes the student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text. ``VRD-Full" is the full model in \cite{VRD}.}
\label{fig:im}
\end{figure}

We show the performance comparisons between our student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text (denoted as ``Our Method") and the full model in \cite{VRD} (denoted as ``VRD-Full") in Figure \ref{fig:im}. We observe that our method significantly outperforms the existing method, especially in the zero-shot (number of training instance is 0) and the few-shot setting (number of training instance is small, e.g., $<10$), which reveals that by distilling linguistic knowledge into a deep model, we can dramatically improve the generalization of our data-driven model, which is hard to achieve by only training it on limited labeled images.



% By properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
% By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (e.g. \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.











==> exp_back_0315.tex <==
\section{Experiments}\label{exp}
% We evaluate our proposed LK-distillation method on the Visual Relationship Detection dataset \cite{VRD}. VRD contains 5,000 images with 70 predicate categories and 100 objects. The training set has 4,000 images with 30,355 relationships and the test set has 1,000 images with 7,638 relationships. The zero-shot subset of the test set consists of 1,877 relationships that occur in the test set but not in the training set. There are three evaluation tasks on VRD dataset:
We evaluate our method on the Visual Relationship Detection \cite{VRD} and Visual Genome \cite{VG} datasets. There are three evaluation tasks:
% 1). \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection.
% 2). \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
% 3). \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\begin{itemize}
\itemsep -1pt
  \item \textbf{Predicate detection}: given an input image and a set of ground truth bounding boxes with corresponding object categories, predict a set of predicates describing each pair of objects. This task evaluates the prediction of predicates without relying on object detection. 
  \item \textbf{Phrase detection}: given an input image, output a phrase \threetup{subj}{pred}{obj} and localize the entire phrase as one bounding box.
  \item \textbf{Relationship detection}: given an input image, output a relationship \threetup{subj}{pred}{obj} and both the subject and the object with their bounding boxes.
\end{itemize}

Both datasets have a zero-shot testing set that contains relationships that never occur in the training data. We also evaluate on the zero-shot sets to demonstrate the generalization improvements brought by linguistic knowledge distillation.

\textbf{Implementation Details.} We use VGG-16 \cite{VGG} to learn the visual representations of the BB-Union of two objects. 
% For phrase and relationship detection, we use R-CNN \cite{Rcnn} for object detection. For fair comparison, we use the proposals provided by \cite{VRD} at test time \footnote{Proposals can be found on {\scriptsize\url{https://github.com/Prof-Lu-Cewu/Visual-Relationship-Detection}}}. 
% For semantic object representation, we try two methods. First, we directly use the confidence scores from object detection as the semantic representations. Second, to leverage the similarity between different combinations of \threetup{subj}{pred}{obj}, 
We use a pre-trained word2vec model to project the subjects and objects into vector space, and the final semantic representation is the weighted average based on the confidence scores of a detection. For the balancing terms, we choose $C=1$ and $\alpha=0.5$ to encourage the student network to mimic the teacher and the ground truth equally.

\textbf{{Evaluation Metric.}} We follow \cite{VRD,UIUC} using Recall@n as the evaluation metric (mAP metric would mistakenly penalize true positives because the annotations in the datasets are not exhaustive).
For two detected objects, there can be multiple predicate predictions with different confident scores. The standard Recall@n metric ranks all predictions for all detected object pairs in an image and chooses the top n predictions to compute the recall. However, instead of computing recall based on all predictions, \cite{VRD} evaluated only the prediction with highest confident score for each object pair. 
By choosing the top prediction, \cite{VRD} made the evaluation more efficient, and forced the diversity of object pairs. 
However, multiple predicates can correctly describe the same object pair, (\eg, when describing a person ``next to" another person, predicates such as ``next to", ``near", ``on the left/right of" are all plausible, but the annotator can only choose one as the ground truth), 
so we believe that a good predicted probability distribution should have large probability for all plausible predicate(s) and probabilities close to 0 for the remaining ones.  Evaluating on only the top prediction per object pair may mistakenly penalize correct predictions because of the annotator's preference or random choice amongst several plausible predicates. 
Thus, we treat the number of chosen predictions per object pair (k) as a hyper-parameter, and report R@n for different $k$'s to compare with other state-of-the-art methods \cite{VRD,UIUC,VisualPhrase}. Since the number of predicates is 70, $k=70$ is equivalent to getting every predictions of two detected objects into evaluation. 
% one can use cross-validation to choose proper k to maximise the performance, to achieve fair comparison with \cite{VRD} and avoid the mistaken penalty because of human annotator's arbitrary predicate selection, 
% 1). \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
% 2). \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 

% \begin{itemize}
% \itemsep -1pt
%   \item \textbf{R@n, k=1}: for each pair of objects, we select the predicate with the highest confidence score per object pair, then evaluate the resulting set. This is for fair comparison with \cite{VRD}.
%   \item \textbf{R@n, k=70}: all 70 predictions of each object pair produced as output, which is the standard way to measure recall, and it reduces the influence of preference of annotators at evaluation time. 
% \end{itemize}

\subsection{Evaluation on VRD Dataset}
\subsubsection{Predicate Prediction}
Since our method models the conditional probability of $P(pred|subj,obj,B_s,B_o,I)$, we first evaluate it given ground truth object detection results, which is the predicate prediction task in \cite{VRD}. 
% Since the labels of objects are given, the confidence score distribution of each detection becomes a one-hot vector. 
Since \cite{UIUC} does not report results of predicate prediction, we compare our results with the methods in \cite{VRD,VisualPhrase}. 

Part 1 of Table \ref{P_VRD} shows the evaluation of linguistic knowledge distillation with different sets of features in our deep neural networks. In addition to the data-driven baseline ``Baseline: U only", we also compare with the baseline that only uses linguistic priors to predict a predicate, which is denoted as ``Baseline: L only". The "Visual Phrases" method \cite{VisualPhrase} trains deformable parts models for each relationship; ``Joint CNN" \cite{Rcnn} trains a 270-way CNN model to predict the subject, object and predicate together. The visual only model and the full model of \cite{VRD} that uses both visual input and language priors are denoted as ``VRD-V only" and ``VRD-Full". S denotes using the student network's output as the final prediction; T denotes using the teacher network's output. T+S denotes that for \twotup{subj}{obj} pairs that occur in the training data, we use the teacher network's output as the final prediction; for \twotup{subj}{obj} pairs that never occur in the training data, we use the student network's output. 

Comparing our baseline, which uses the same visual representation (BB-Union) as \cite{VRD}, and the ``VRD-V only" model, our huge recall improvement (R@100/50, k=1 increases from 7.11\% \cite{VRD} to 34.82\%) reveals that the end-to-end training with soft-max prediction outperforms extracting features from a fixed CNN + linear model method in \cite{VRD}, highlighting the importance of fine-tuning. In addition, adding the semantic representation and the spatial features improves the predictive power and generalization of the data-driven model. \footnote{More analysis on using different combinations of features can be found in the supplementary materials.}



\begin{table}[]
\centering
\scriptsize
\setlength{\tabcolsep}{3.5pt} 
\caption{Predicate Detection on VRD Testing Set: ``U" is the union of two objects' bounding boxes; ``SF" is the spatial representation; ``W" is the word-embedding based semantic representations; ``L" means using LK distillation; ``S" is the student network; ``T" is the teacher network and ``S+T" is the combination of them. Part 1 uses the training images in VRD dataset; Part 2 uses the training images in VRD \cite{VRD} and all images of Visual Genome (VG) \cite{VG} dataset.}
\label{P_VRD}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{@{}l}{ } & R@100/50\tablefootnote{In predicate detection task, R@100,k=1 and R@50,k=1 are exactly equivalent because there aren't enough ground truth objects in the image to produce more than 50 predictions, just as in \cite{VRD}.}     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 1.91             & -           & -    & - & - & -      \\
Joint CNN  \cite{Rcnn}           & 2.03             & -           & -    & - & - & -      \\

VRD-V only \cite{VRD}                                    & 7.11      & 37.20
\tablefootnote{The results of Recall when k=70 are not reported in \cite{VRD}. To show the improvement of our method with different k's we calculate those recall values using their code. The same for Table \ref{Detection} and \ref{Detection_Zero}.}          
& 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline

Baseline: U only                                       & 34.82     & 83.15       & 70.02    & 12.75     & 69.42       & 47.84   \\
Baseline: L only                                       & 51.34     & 85.34       & 80.64    & 3.68      & 18.22       & 8.13   \\\hdashline
U+W                             & 37.15     & 83.78       & 70.75   & 13.44     & 69.77       & 49.01    \\
U+W+L:S               & 42.98     & 84.94       & 71.83  & 13.89       & 72.53       & 51.37     \\
U+W+L:T               & 52.96     & 88.98       & 83.26   & 7.81          & 40.15      & 32.62   \\\hdashline
U+SF                 &36.33           & 83.68       & 69.87  & 14.33     & 69.01       & 48.32    \\
U+SF+L:S                       & 41.06     & 84.81       & 71.27    & 15.14          & 72.72       & 51.62  \\
U+SF+L:T               & 51.67     & 87.71       & 83.84     & 8.05          & 41.51       & 32.77    \\ \hdashline
U+W+SF                   & 41.33     & 84.89       & 72.29  & 14.13         & 69.41       & 48.13    \\
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & \textbf{16.98}       & \textbf{74.65}       & \textbf{54.20}    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81    \\
U+W+SF+L: T+S    & \textbf{55.16}     & \textbf{94.65}       & \textbf{85.64}    & -          & -       & -  \\
\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}
                                              & & &  &                      \\
Baseline: U                                           & 36.97     & 84.49  & 70.19   & 13.31     & 70.56  & 50.34     \\
U+W+SF                     & 42.08     & 85.89       & 72.83   & 14.51          & 70.79       & 50.64     \\
U+W+SF+L: S             & 48.61      & 87.15       & 75.45    & 17.16          & 75.26       & 55.41     \\
U+W+SF+L: T             & 54.61     & 90.09       & 82.97       & 9.23          & 43.21       & 33.40  \\
U+W+SF+L: T+S               & 55.67     &95.19      & 86.14    & -          & -       & -    \\
\bottomrule
\end{tabular}
\end{table}



\begin{figure*}[!h]
\centering     %%% not \center
\subfigure[Seen relationships]{\label{v}\includegraphics[width=140mm]{images/visual_1.pdf}}

\subfigure[Zero-shot Relationships]{\label{vz}\includegraphics[width=140mm]{images/visual_2.pdf}}
\caption{Visualization of predicate detection results: ``Data-driven" denotes the baseline using BB-Union; ``LK only" denotes the baseline using only the linguistic knowledge without looking at the image; ``Full model student" denotes the student network with U+W+SF features; ``Full model teacher" denotes the teacher network with U+W+SF features.}
\end{figure*}



\begin{table*}[t]
\centering
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\label{Detection}
% \footnotesize
\scriptsize
\setlength\tabcolsep{3.5pt}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
& \multicolumn{6}{c|}{\bf Phrase Detection}                                               & \multicolumn{6}{|c}{\bf Relationship Detection}                                        \\ 
% \textbf{Part 1: VRD only} 
& R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,                  & R@100,                 & R@50,  & R@100,                 & R@50,                  & R@100,                 & R@50,                \\
& k=1                    & k=1                    & k=10                   & k=10                   & k=70                    & k=70                    & k=1                   & k=1     & k=10                   & k=10                    & k=70                   & k=70              \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&\\
Visual Phrases \cite{VisualPhrase}       & 0.07             & 0.04           & -    & - & - & -   & -& -& -& -& -   \\
Joint CNN  \cite{Rcnn}           & 0.09             & 0.07           & -    & - & - & - & 0.09    & 0.07 & - & -& -    & -      \\
% VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & -                      & -       & -                      & -               &14.70                  & 13.86                  & -                      & -            & -                    & -          \\
VRD - V only  \cite{VRD}           & 2.61             & 2.24           & -    & - & - & - & 1.85    & 1.58 & - & -& -    & -      \\
VRD - Full \cite{VRD}        & 17.03                  & 16.17                  & 25.52                      & 20.42       & 24.90                      & 20.04               & 14.70                  & 13.86                  & 22.03                      & 17.43            & 21.51                    & 17.35          \\
Linguistic Cues   \cite{UIUC}       & -                      & -                      & 20.70                  & 16.89                & --                      & --  & --                      & --                      & 18.37                  & 15.08         & --                      & --         \\ \hdashline
U+W+SF+L: S      & 19.98 & 19.15 & 25.16 & 22.95 & 25.54	& 22.59 & 17.69 & 16.57 & 27.98 & 19.92 &28.94	&20.12\\
U+W+SF+L: T      & 22.97 & 22.06 & 29.14 & 25.96 &29.09	&25.86 & 19.81 & 18.67 & 29.36 & 21.89 &31.06	&21.96\\
U+W+SF+L: T+S  & \textbf{23.47} & \textbf{22.34} & \textbf{29.76} & \textbf{26.47} &\bf29.43	&\bf26.32 & \textbf{20.25} & \textbf{19.01} & \textbf{29.89} & \textbf{22.56} &\bf 31.89	&\bf22.68\\

\midrule

\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 20.32 & 19.96 & 25.71 & 23.34 & 25.97	& 22.83 & 18.32 & 16.98 & 28.24 & 20.15 &29.85	&21.88\\
U+W+SF+L: T      & 23.32 & 22.56 & 29.89 & 26.34 &29.92	&26.15 & 20.04 & 18.91 & 29.95 & 22.42 &31.74	&22.64\\
U+W+SF+L: T+S     & 23.96 & 22.84 & 30.13 & 26.73 &30.01	&26.58 & 20.56 & 19.38 & 30.45 & 22.84 &32.56	&23.18\\ 
\bottomrule

\end{tabular}
\end{table*}



\begin{table*}[t]
\centering
% \footnotesize
\scriptsize
\caption{Phrase and Relationship Detection: Distillation of Linguistic Knowledge - Zero Shot. We use the same notations as in Table \ref{P_VRD}.}\vskip 3pt
\setlength\tabcolsep{3.8pt}
\label{Detection_Zero}
\begin{tabular}{@{}lcccccc|cccccc@{}}
\toprule
                   & \multicolumn{6}{c|}{\bf Phrase Detection}                                                            & \multicolumn{6}{|c}{\bf Relationship Detection}                                                      \\ 
                   & R@100,                & R@50,                 & R@100,                 & R@50,                  & R@100,                & R@50,                 & R@100,                 & R@50,    & R@100,                & R@50,                 & R@100,                 & R@50,              \\
                   & k=1                   & k=1                   & k=10                   & k=10                   & k=70                   & k=70                   & k=1                   & k=1   & k=10                   & k=10                   & k=70                   & k=70                \\\midrule
\multicolumn{3}{@{} l}{Part 1: Training images VRD only}&&&&&&&&&&\\

% VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & -                     & -    & -                      & -                  & 3.52                  & 3.13                  & -                      & -      & -                     & -                \\
VRD - V only  \cite{VRD}           & 1.12             & 0.95           & -    & - & - & - & 0.78    & 0.67 & - & -& -    & -      \\
VRD - Full \cite{VRD}   & 3.75                  & 3.36                  & 12.57                      & 7.56    & 12.92                      & 7.96                  & 3.52                  & 3.13                  & 11.46                      & 7.01      & 11.70                      & 7.13                \\
Linguistic Cues  \cite{UIUC}   & -                     & -                     & 15.23                  & 10.86    & -                      & -              & -                     & -                     & 13.43                  & 9.67   & -                      & -                \\\hdashline
U+W+SF+L: S   & \textbf{10.89} & \textbf{10.44} & \textbf{17.24} & \textbf{13.01} &\bf 17.24	&\bf 12.96 & \textbf{9.14} & \textbf{8.89} & \textbf{16.15} & \textbf{12.31} &\bf 15.89	&\bf 12.02\\ 	
U+W+SF+L: T      & 6.71 & 6.54 & 11.27 & 9.45 &9.84	&7.86 & 6.44 & 6.07 & 9.71 & 7.82 &10.21	&8.75\\
\midrule
   
\multicolumn{3}{@{} l}{Part 2: Training images VRD + VG}&&&&&&&&&&\\
U+W+SF+L: S      & 11.23 & 10.87 & 17.89 & 13.53 & 17.88	& 13.41 & 9.75 & 9.41 & 16.81 & 12.72 &16.37	&12.29\\
U+W+SF+L: T      & 7.03 & 6.94 & 11.85 & 9.88 &10.12	&8.97 & 6.89 & 6.56 & 10.34 & 8.23 &10.53	&9.03\\

\bottomrule


\end{tabular}
\end{table*}

To demonstrate the effectiveness of LK-distillation, we compare the results of using different combinations of features with/without using LK-distillation. In Part 1 of Table \ref{P_VRD}, for fair comparison with existing methods, we train and test our model on only the VRD dataset, and use the training annotation as our linguistic knowledge. 
First, we observe that the linguistic knowledge (``Baseline: L only") itself has a strong predictive power and it outperforms the state-of-the-art method \cite{VRD} by a large margin (\eg, 51.34\%  vs. 47.87\% for R@100/50, k=1 on the entire VRD test set), which implies the knowledge we distill in the data-driven model is reliable and discriminative. 
However, since, some \twotup{subj}{obj} pairs in the zero-shot test set never occur in the linguistic knowledge extracted from the VRD train set, trusting only the linguistic knowledge without looking at the images leads to very poor performance on the zero-shot set of VRD, which explains the poor generalization of ``Baseline: L only" method and addresses the need for combining both data-driven and knowledge-based methods as the LK-distillation framework we propose does.

The benefit  of LK distillation is visible across all feature settings: the data-driven neural networks that absorb linguistic knowledge (``student" with LK) outperform the data-driven models significantly (\eg, R@100/50, k=1 is improved from 37.15\% to 42.98\% for ``U+W" features on the entire VRD test set).
On the entire test set, for all feature settings, the teacher networks still outperform the students by a large margin (rather than converging in performance). 
There are two possible reasons: one is that the student networks absorb only partial knowledge rather than all of it due to the limited number of teacher-student pairs in the training data; the other is that although the linguistic prior is powerful, it may still be misleading in some cases (R@100/50, k=1 is 51.34\% for LK only baseline, which is still far from perfect). Since the student network not only mimics the teacher network's behavior but is also trained with the one-hot ground truth object labels (we set $\alpha=1$ to make the effect of teacher network and ground truth labels equivalent), when there is a conflict between LK and ground truth labels, the student network achieves a balance between them. 
We also observe consistent improvement of the recall on the zero-shot test set of data-driven models that absorb the linguistic knowledge. The student networks with LK-distillation yield the best generalization, and outperform the data-driven baselines and knowledge only baselines by a large margin.
% (\eg, 15.53\% vs. 11.72\% for R@100/50, k=1 for ``U+W+SF+LK: S" method). 

Unlike \cite{hinton,eric1,eric2}, where either the student or the teacher network is the final output, both the student and teacher in our framework are used, since they each have their own advantages. The best predictive power is achieved when we combine them together: we use the teacher network to predict the predicates whose \twotup{subj}{obj} pairs occur in the training data, and use the student network for the remaining ones. The setting ``U+W+SF+LK: T+S" achieves the best performance. 
% One interesting finding is that when we set k=70 to calculate recall, our teacher+student method achieves 93.55\% R@100 and 84.34\% R@50. According to \cite{VRD}'s human evaluation, human obtained a 98.1\% R@50. Although there is still a gap between our model and the human model, our method shows a promise toward approaching human level perception by combining data-driven models and external knowledge. 
Visualizations of the different methods are shown in Figure \ref{v} and \ref{vz}. 

\subsubsection{Phrase and Relationship Detection}
To enable a fully automatic method for phrase detection and relationship detection, we train a Fast R-CNN detector \cite{fastRCNN} for object detection tasks. Given the confidence scores of detected each object, we use the weighed word2vec vectors as the semantic object representation, and extract spatial features from each detected bounding box pairs. We then use the pipeline in Figure \ref{fig:system} to obtain the predicted predicate distribution for each pair of objects. According to Eq. \eqref{decompose}, we use the product of the predicate distribution and the confidence scores of the subject and object as our final prediction results. To compare with \cite{VRD}, we report R@n, k=1 for both phrase detection and relationship detection. For fair comparison with \cite{UIUC} (denoted as ``Linguistic Cues"), we choose k=10 as they did to report recall. In addition, we report the full recall measurement k=70. Evaluation results on the entire dataset and the zero-shot setting are shown in Part 1 of Tables \ref{Detection} and \ref{Detection_Zero}. Our method outperforms the state-of-the-art methods in \cite{VRD} and \cite{UIUC} significantly on both entire testing set and zero-shot setting. The observations about student and teacher networks are consistent with predicate prediction evaluation. 
% Additionally, when comparing the results of predicate and relationship prediction, the large performance gain (5.85 \% vs. 17.30\% for R@100/50, k=1) indicates that the high-level relationship detection task is highly limited by the fundamental object detection task.

\subsection{Evaluation on Visual Genome Dataset}

We also evaluate our method on the Visual Genome dataset (VG) \cite{VG}, which is the largest dataset that has visual relationship annotations, on the predicate detection task. We randomly split the VG dataset into training (88,077 images) and testing set (20,000 images) and select the relationships that have predicates and objects in the categories of VRD dataset. We conduct a similar evaluation on the dataset (99,864 relationship instances in training and 19,754 in testing; In the testing set, 2,056 relationships instance are never seen in the training data). We use the linguistic knowledge extracted from VG and report the predicate prediction results in Table \ref{VG}. 

Not surprisingly, we observe similar behavior as our experiments on the VRD dataset---LK distillation manages to regularize the deep model and improve its generalization. We conduct another experiment in which images from Visual Genome dataset augment the training set of VRD and evaluate on the VRD test set. From the Part 2 of Tables \ref{P_VRD}, \ref{Detection} and \ref{Detection_Zero}, we observe that training with more data leads to only marginal performance improvement of almost all baselines and proposed methods. However, for all experimental settings, with more data, our LK distillation framework still brings significant improvements, and the combination of the teacher and student networks still yields the best performance, which reveals that incorporating additional knowledge is more beneficial than collecting more data\footnote{Details can be found in the supplementary materials.}. 

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on Visual Genome Dataset. Notations are the same as in Table \ref{P_VRD}.}
\label{VG}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{c}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{c}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
U                    & 37.81    & 82.05    & 81.41    & 7.54     & 81.00    & 65.22   \\
U+W+SF               & 40.92    & 86.81    & 84.92    & 8.66     & 82.50    & 67.72   \\
U+W+SF+L: S         & 49.88    & 91.25    & 88.14    & \textbf{11.28}    & \textbf{88.23}    & \textbf{72.96}   \\
U+W+SF+L: T         & 55.02    & 94.92    & 91.47    & 3.94     & 62.99    & 47.62   \\
U+W+SF+L: T+S       & \textbf{55.89}    & \textbf{95.68}    & \textbf{92.31}    & -        & -        & -       \\ \bottomrule
\end{tabular}
\end{table}



\subsection{Distillation with External Knowledge}
The above experiments show the benefits of extracting linguistic knowledge from internal training annotations and distilling them in a data-driven model. 
% However, utilizing only the training annotations may not bring in large improvement for relationships whose \twotup{subj}{obj} pairs never occur in the training data. 
However, training annotations only represent a small portion of all possible relationships and do not necessarily represent the real world distribution, which has a long tail.
For those unseen long-tail relationships in the VRD dataset, we extract the linguistic knowledge from external sources: the Visual Genome annotations and Wikipedia, whose domain is much larger than any annotated visual dataset. 
In Table \ref{VRD_use_VG_Stat}, we show the predicate detection results on the VRD test set using our linguistic knowledge distillation framework with different sources of knowledge. 
From Part 2 and Part 4 of Table \ref{VRD_use_VG_Stat}, we observe that using only the external knowledge, especially the very noisy knowledge obtained from Wikipedia, leads to bad performance. 
However, interestingly, although the external knowledge can be very noisy (Wikipedia) or have a different distribution when compared with the VRD dataset (Visual Genome), the performance of the teacher network using such external knowledge is much better than that restricted to the VRD training dataset (Part 1). 
This finding suggests that by properly distilling the external knowledge, our framework can obtain both good predictive power on the seen relationships and better generalization on the unseen ones. 
% To help the data-driven model properly absorb the external knowledge, we conduct a two-step knowledge distillation: at the first several training epoches, we only allow the student to absorb the knowledge from training annotations to first establish a good data-driven model. 
% After that, we start distilling the external knowledge together with the knowledge extracted from training annotations weighted by the balancing term C as shown in Eq. \eqref{objective}. 
% The weights Cs are chosen by cross-validation on a validation set we select from the training set (1,000 out of 4,000 images). 
% We observe that when the weight of external knowledge increases, the performance of the entire validation set decreases, so we select the weight that maximize the performance on the zero-shot validation. 
Evaluation results of combining both internal and external linguistic knowledge are shown in Part 3 and Part 5 of Table \ref{VRD_use_VG_Stat}. We observe that by distilling external knowledge with the internal one, we improve the generalization significantly (\eg, LK from Wikipedia boosts the recall to 19.17\% on the zero-shot set) while maintaining good predictive power on the entire test set.

\begin{table}[!h]
\centering
\scriptsize
\setlength{\tabcolsep}{3.6pt} 
\caption{Predicate Detection on VRD Testing Set: External Linguistic Knowledge. Part 1 uses the LK from VRD dataset; Part 2 uses the LK from VG dataset; Part 3 uses the LK from both VRD and VG dataset. Part 4 uses the LK from parsing Wikipedia text; Part 5 uses the LK from from both VRD dataset and Wikipedia. Notations are the same as as in Table \ref{P_VRD}. }
\label{VRD_use_VG_Stat}
\begin{tabular}{@{}lccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c}{Entire Set} & \multicolumn{3}{c}{Zero-shot} \\ \midrule
\multicolumn{1}{l}{} & R@100/50     & R@100    & R@50     & R@100/50     & R@100    & R@50    \\
\multicolumn{1}{l}{} & k=1      & k=70      & k=70     & k=1      & k=70      & k=70    \\\midrule
Part 1 LK: VRD  & \multicolumn{3}{c|}{} \\
VRD-V only \cite{VRD}                                    & 7.11      & 37.20           & 28.36       & 3.52      & 32.34           & 23.95   \\ 
VRD-Full \cite{VRD}                                & 47.87     & 84.34           & 70.97       & 8.45      & 50.04           & 29.77   \\\hdashline
U+W+SF+L: S            & 47.50      & 86.97       & 74.98  & 16.98       & 74.65       & 54.20    \\
U+W+SF+L: T          & 54.13     & 89.41       & 82.54   & 8.80           & 41.53       & 32.81     \\\midrule
Part 2 LK: VG & \multicolumn{3}{c|}{} \\
U+W+SF+L: S         & 45.00   & 81.64    & 74.76    & 16.88   & 72.29    & 52.51   \\
U+W+SF+L: T         & 51.54    & 87.00   & 79.70    & 11.01    & 54.66    & 45.25   \\\midrule
\multicolumn{2}{@{} l}{Part 3 LK: VRD+VG} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.21    & 87.76   & 76.51    & 17.21    & 74.89   & 54.65   \\
U+W+SF+L: T         & \textbf{54.82}    & \textbf{90.63}    & \textbf{83.97}    & 12.32     & 47.22    & 38.24  \\\midrule

\multicolumn{2}{@{} l}{Part 4 LK: Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 36.05    & 77.88   & 68.16    & 11.80   & 64.24    & 49.19   \\
U+W+SF+L: T         & 30.41    & 69.86   & 60.25    & 11.12    & 63.58    & 44.65  \\\midrule

\multicolumn{2}{@{} l}{Part 5 LK: VRD+Wiki} & \multicolumn{2}{c|}{} \\
U+W+SF+L: S         & 48.94   & 87.11   & 77.79    & \textbf{19.17}    & \textbf{76.42}    & \textbf{56.81}   \\
U+W+SF+L: T         & 54.06    & 88.93   & 81.78    & 9.65     & 42.24   & 34.61  \\\bottomrule
\end{tabular}
\end{table}

\begin{figure}[!t]
\centering
  \includegraphics[width=60mm]{images/I_N}
  \caption{Performance with varying sizes of training examples. ``Our Method" denotes the student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text. ``VRD-Full" is the full model in \cite{VRD}.}
\label{fig:im}
\end{figure}

We show performance comparisons between our student network that absorbs linguistic knowledge from both VRD training annotations and the Wikipedia text (denoted as ``Our Method") and the full model in \cite{VRD} (denoted as ``VRD-Full") in Figure \ref{fig:im}. We observe that our method significantly outperforms the existing method, especially for the zero-shot (relationships with 0 training instance) and the few-shot setting (relationships with few training instances, \eg, $<10$), which reveals that by distilling linguistic knowledge into a deep model, we can dramatically improve the generalization of our data-driven model, which is hard to achieve by only training it on limited labeled images.



% By properly distilling the external knowledge, we manage to obtain better performance on both entire and zero-shot set. Especially when we distill the knowledge from Wikipedia, we obtain significant improvement of the model's generalization. 
% By analyzing the zero-shot testing data, we found that tuples we mine from Wikipedia (\eg \threetup{motorcycle}{has}{engine}), \threetup{mountain}{by}{road})) help the data-driven model correctly predict the predicates in zero-shot set.











==> intro_backup.tex <==
\section{Introduction}
Detecting visual relationships from images is a central problem in image understanding and a variety of high level computer vision applications, such as text-based image retrieval \cite{Johnson_2015_CVPR,li2016_3dscenefromtext}, visual question answering \cite{Sadeghi_2015_CVPR} and referring expression understanding \cite{varun}. Relationships are commonly defined as tuples of subject (\textit{subj}), predicate (\textit{pred}) and object (\textit{obj}) in natural language processing \cite{nlp1,nlp2,nlp3}. Similarly, visual relationships represent the visually observable interactions between subject and object \twotup{subj}{obj} pairs, such as \threetup{person}{ride}{horse} \cite{VRD}. 

\begin{figure}[!t]
\centering
  \includegraphics[width=\linewidth]{images/system.pdf}
  \caption{Linguistic Knowledge Distillation Framework. We extract linguistic knowledge from training annotations and other public text corpus (green box), then construct a teacher network to distill the knowledge into an end-to-end deep neural network (student) that predicts visual relationships from visual and semantic representations (red box). GT is the ground truth label. ``+" is the concatenation operator.}
\label{fig:system}
\end{figure}

Recently, Lu \etal \cite{VRD} introduced the visual relationship dataset (VRD) to study learning of a large number of visual relationships from images. 
% Since it is difficult to collect a sufficiently large number of training images for all possible \threetup{subj}{pred}{obj} combinations, 
Lu \etal predict the predicates independent from the subjects and objects, and use the product of their scores to predict relationships present in a given image using a linear model:
\begin{equation}
\label{VRD_decompose}
V(R|I)=P(subj)(\mathbf{w}^\text{T}CNN(I_{\text{union}})+b)P(obj)
\end{equation}
where $CNN(I_{\text{union}})$ are the CNN features of a cropped image that contains the union of the two object bounding boxes. 
The results in \cite{VRD} suggest that predicates cannot be predicted reliably with only visual module, even when the ground truth categories and bounding boxes of the subject and object are given (\cite{VRD} reports Recall@100 of only 7.11\% for their visual module). In \cite{VRD}, although the cropped image includes the subject and object, predicates are predicted without any knowledge about the object categories or relative locations. 
Thus, we propose a standard probabilistic model to predict the predicate name jointly with the subject and object names and their relative spatial arrangement:
\begin{align}
\label{decompose}
P(R|I) =P(pred|I_{\text{union}},subj,obj)P(subj)P(obj).
\end{align}

While the proposed method models visual relationships more accurately, the model's parameter space is also enlarged because of the large variety of relationship tuples. This leads to the visual data challenge of insufficient image data. The straightforward---but very costly---solution is to collect and annotate a larger image dataset that can be used to train this model. Due to the long tail distribution of relationships, it is hard to collect enough training images for all relationships. To make the most of available training images, we leverage linguistic knowledge (LK) to regularize the deep neural network. One way to obtain linguistic knowledge is to compute conditional probability of $P(pred|subj,obj)$ in the training annotations, which effectively models the strong correlation between \twotup{subj}{obj} pairs and predicates (e.g., if the subject and object were ``cup" and ``table", the predicate would be very likely to be ``on"). We denote the linguistic knowledge obtained from training annotations ``internal knowledge".
% in the training set to regularize the deep neural network. 

% Another challenge is the linguistic data challenging. 
Since the number of \threetup{subj}{pred}{obj} combinations is too large to be covered in a dataset of annotated images, the internal statistics (e.g., statistics of the VRD dataset) only capture a small portion of the knowledge in nature.
To address that problem, we collect external linguistic knowledge ($P(pred|subj,obj)$) from public texts on the Internet (Wikipedia) and distill it into the data-driven model. 
This external knowledge is extracted from a much larger and unconstrained domain and consists of statistics about which word humans commonly use to describe the relationship between a given subject and object pair, which hopefully includes unseen \twotup{subj}{obj} pairs in our training data. Although the external knowledge is more general, it can be very noisy (e.g., due to errors in linguistic parsing). Thus we combine the internal and external knowledge in a (multi-) teacher-student knowledge distillation framework shown in Figure \ref{fig:system}. 

We adopt a teacher-student framework \cite{eric1,eric2}, where the output of the standard deep vision pipeline, called the \textit{student} network, is augmented with the output of a model that uses the linguistic knowledge to score solutions, and their combination is called the \textit{teacher} network. 
An additional term is then added to the standard loss function that penalizes divergence between student and teacher outputs. 
The objective is formulated so that the student not only learns to predict the correct one-hot ground truth labels but also to mimic the teacher's soft belief between predicates.

Our main contribution is that we exploit the role of different visual and linguistic representations in visual relationship detection and use internal and external linguistic knowledge to regularize the learning process of an end-to-end deep neural network to significantly enhance its predictive power and generalization. We evaluate our contributions on the VRD \cite{VRD} and Visual Genome (VG) \cite{VG} datasets. For fair comparison, our method that utilizes only internal linguistic knowledge significantly outperforms the state-of-the-art methods \cite{VRD,UIUC} (e.g. we achieve a Recall@100 of 29.56\% vs. 18.37\% in \cite{UIUC} on VRD dataset for relationship detection).
With linguistic knowledge distillation, our method outperforms the pure data-driven baseline significantly (by 22.23\% Recall@100 for predicate detection). Our student network obtains better generalization ability, especially in the zero-shot setting with unseen relationships (we improve predicate detection (Recall@100) from 8.45\% \cite{VRD} to 15.53\%). Our experiments on the Visual Genome dataset shows that the while the improvements due to training set size are minimal, improvements due to the use of LK remain is large, implying that with current dataset sizes, it is more fruitful to incorporate additional knowledge (e.g., LK) than to increase the dataset size.
Our evaluation of the combination of the internal and external linguistic knowledge suggests that we can train a student network that benefits from internal linguistic statistics for common visual relationships and from external statistics for long-tail relationships.



